The geodesic edge center of a simple polygon

The geodesic edge center of a polygon is a point c inside the polygon that minimizes the maximum geodesic distance from c to any edge of the polygon, where geodesic distance is the shortest path distance inside the polygon. We give a linear-time algorithm to find a geodesic edge center of a simple polygon. This improves on the previous O(n log n) time algorithm by Lubiw and Naredla [European Symposium on Algorithms, 2021]. The algorithm builds on an algorithm to find the geodesic vertex center of a simple polygon due to Pollack, Sharir, and Rote [Discrete & Computational Geometry, 1989] and an improvement to linear time by Ahn, Barba, Bose, De Carufel, Korman, and Oh [Discrete & Computational Geometry, 2016]. The geodesic edge center can easily be found from the geodesic farthest-edge Voronoi diagram of the polygon. Finding that Voronoi diagram in linear time is an open question, although the geodesic nearest edge Voronoi diagram (the medial axis) can be found in linear time. As a first step of our geodesic edge center algorithm, we give a linear-time algorithm to find the geodesic farthest-edge Voronoi diagram restricted to the polygon boundary.

==> SoCG-100_Intro.tex <==
\section{Introduction}\label{section:introduction}

The most basic ``center'' problem is Sylvester's problem: given $n$ points in the plane, find the smallest disc that encloses the points. The center of this disc is a point that minimizes the maximum distance to any of the given points.
We consider a center problem that differs in two ways from Sylvester's problem. First, the domain is a simple polygon and the distance measure is not Euclidean distance, but rather the shortest path, or ``geodesic'' distance inside the polygon.
Second, the sites are not points but rather the edges of the polygon.  More precisely, the problem is to find, given a simple polygon in the plane, the \defn{geodesic edge center}, which is a point in the polygon that minimizes the maximum geodesic distance to a polygon edge. 
See Figure~\ref{fig:center-example}.
More formally, let $E$ be the set of edges of the polygon $P$, and for point $p \in P$ and edge $e \in E$, define \defn{$d(p,e)$} to be the geodesic distance from $p$ to $e$.  
\changed{Define the \defn{geodesic radius} of a point $p \in P$ to be $r(p) := \max \{d(p,e): e \in E\}$.
Then the \defn{geodesic edge center} is a point $p \in P$ that minimizes
$r(p)$.}

\begin{figure}[htb]
  \centering
  \includegraphics[width=.65\textwidth]{RS_figures/EdgeCenter-cropped.pdf}
  \caption{Point $c$ is the edge center of this polygon.
  Edges $e, e', e''$ (in blue)
  are geodesically farthest
  from $c$---the geodesic paths (in red) from $c$ to these edges all
have the same length.}
\label{fig:good_four_cell}
\label{fig:center-example}
\end{figure}

Our main result is a linear-time algorithm to find the geodesic edge center of a simple $n$-vertex polygon.  This improves the previous $O(n \log n)$ time algorithm by Lubiw and Naredla~\cite{lubiw2021visibility}.
The algorithm follows the strategies used to find the geodesic \emph{vertex} center, which is a point in the polygon that minimizes the maximum geodesic distance to a polygon vertex.  
In 1989, Pollack, Sharir and Rote~\cite{pollack_sharir} gave an $O(n \log n)$ time algorithm for the geodesic vertex center problem.  A main tool---which is used in all subsequent algorithms---is
a linear time \emph{chord oracle} that finds, given a chord, which side of the chord contains the center. 
In 2016, Ahn, Barba, Bose, De Carufel, Korman, and Oh~\cite{linear_time_geodesic} improved the runtime for the geodesic vertex center to $O(n)$.  
Their most important new contribution is the use of $\epsilon$-nets to perform a divide-and-conquer search. 
Our algorithm follows the approach of Ahn et al., modified to deal with farthest edges rather than farthest vertices.  We simplify some aspects and we repair some %
errors in their approach.  
\newchanged{The edge center problem is more general than the vertex center problem via the reduction of splitting each vertex into  two vertices joined by a very short edge.}
\remove{Our result is more general, since farthest vertices can be converted to farthest edges by 
adding a small edge at each vertex.}


In general, the center of a set of sites can be determined from the farthest Voronoi diagram of those sites, but computing the Voronoi diagram can be more costly. 
As the first step of 
our center algorithm we give a \reviewerchange{linear-time} algorithm to compute the \reviewerchange{geodesic farthest-edge} Voronoi diagram restricted to the boundary of the polygon. 
\changed{Computing the whole \reviewerchange{geodesic farthest-edge} Voronoi diagram in linear time is an open problem.}


\remove{
\attention{I think the next paragraph must either be removed or modified! Khramtcova and Papadopoulou don't note anywhere the case for a convex polygon but it works in linear expected time. We can get the expected time part down to output sensitive linear + use aurenhammer et al. to get a deterministic \reviewerchange{linear-time algorithm} when the size of the Voronoi diagram is $O(\frac{n}{\log n})$.}
\anna{OK, we should remove this part.  Also, I don't see `output sensitive linear time' since it takes $O(n)$ to compute the Voronoi diagram on $\partial P$---you can't ignore that runtime.  I think we should just drop the whole thing.}
\anurag{removed.}
}





\subparagraph*{Background on Centers and Farthest Voronoi Diagrams.} 

\changed{
Megiddo~\cite{megiddo_linear} gave a linear time  algorithm to find the center of a set of points in the plane (Sylvester's problem) using his ``prune-and-search'' technique, which is used in the final stages of all geodesic center algorithms.
However, computing the farthest Voronoi diagram of points in the plane takes $\Theta(n \log n)$ time~\cite{shamos1975closest}.
}



\remove{
The center of a set of points in the plane (Sylvester's problem) 
can be determined from the farthest point Voronoi diagram---the center is a vertex of the Voronoi diagram unless the center has only two farthest points, in which case it lies on an edge of the Voronoi diagram.
Shamos and Hoey~\cite{shamos1975closest} gave an $O(n \log n)$ time algorithm to find the farthest point Voronoi diagram and the center. 
There is an $\Omega(n \log n)$ lower bound for finding Voronoi diagrams of points in the plane, but the center problem is strictly easier---Megiddo~\cite{megiddo_linear} used his ``prune-and-search'' technique to give a \reviewerchange{linear-time algorithm} to find the center of a set of points in the plane. 
It turns out that all algorithms for geodesic center problems end up using Megiddo's prune-and-search techniques in the last stages.  
}

Our problem involves distances that are geodesic rather that Euclidean, and sites that are segments (edges) rather than points. \changed{These have been studied separately, although there is almost no work
combining them.}

For Euclidean distances, 
Megiddo's method extends to \reviewerchange{linear-time algorithm}s to find the center of %
line segments or lines in the plane~\cite{bhattacharya1994optimal}.
The farthest Voronoi diagram of segments in the plane was considered by Aurenhammer et al.~\cite{aurenhammer2006farthest},
who called it a
``stepchild in
the vast Voronoi diagram literature''.  
They gave an $O(n \log n)$ time algorithm which was improved to output-sensitive time $O(n \log h)$, where $h$ is the number of faces of the diagram~\cite{papadopoulou2013farthest}.

\remove{
There are algorithms 
to find the Euclidean center of more general sites such as convex polygons~\cite{jadhav1996optimal}, and to find the smallest disc that \emph{contains} a set of discs~\cite{megiddo_spanned_ball} which can be viewed as a center problem for points with additive weights, and is one of the ingredients in the algorithms for finding the vertex center of a polygon.
With regard to Voronoi diagrams, 
there is an algorithm to find 
the farthest Voronoi diagram of convex polygons in the plane~\cite{cheong2011farthest},
and more generalizations can be found in 
the book by Aurenhammer et al.~\cite{aurenhammer2013voronoi}.
}



For geodesic 
distances with point sites Ahn et al. gave 
a \reviewerchange{linear-time algorithm} to find the geodesic center of the vertices of a polygon~\cite{linear_time_geodesic}.
The corresponding farthest Voronoi diagram 
can be found in time $O(n \log \log n)$~\cite{oh2020geodesic}, and in expected linear time~\cite{barba2019optimal}. 
More generally, for $m$ points inside an $n$-vertex polygon, an algorithm to find their farthest Voronoi diagram 
was first given by Aronov et al.~\cite{aronov1993farthest} with run-time $O((n+m)\log (n+m))$, and improved in a sequence of papers~\cite{oh2020geodesic,barba2019optimal,oh2020voronoi}, culminating in an optimal run time of   
$O(n + m \log m)$~\cite{wang2021optimal}. \changed{This is also the best-known bound for finding the center of $m$ points in a simple polygon.}
For sites more general than point sites inside a polygon, the only result we are aware of is %
an $O((n+m) \log (n+m))$ time algorithm to find the geodesic center of $m$ \emph{half-polygons}~\cite{lubiw2021visibility}, 
with edges being a special case. 

Finally, we mention a curious difference between nearest and farthest site Voronoi diagrams of edges
in a polygon.
The nearest Voronoi diagram of the edges of a polygon is the medial axis, 
one of the most famous and useful Voronoi diagrams.  The medial axis can be found in linear time~\cite{chin1999finding}.
By contrast,
the \emph{farthest} Voronoi diagram of edges in a polygon has received virtually no attention,
\changed{except for a convex polygon (which avoids geodesic issues)
where there is an $O(n \log n)$ time algorithm~\cite{drysdale2008nlogn}, and a recent 
expected \reviewerchange{linear-time algorithm}~\cite{khramtcova2014expected}.
}

\remove{
\subparagraph*{Techniques and Our Contributions.}
Our algorithm to find the geodesic edge center of a polygon has two phases.  In the first phase we find the \reviewerchange{geodesic farthest-edge} Voronoi diagram restricted to the polygon boundary.  In the second phase we reduce the problem to finding a point in the polygon that minimizes the upper envelope of a linear number of easy-to-compute
\changed{convex} functions each defined on a triangle inside the polygon. 
That problem is then solved using a divide-and-conquer algorithm based on $\epsilon$-nets
\changed{and Megiddo's prune and search techniques}.  
A more detailed overview of our algorithm can be found in Section~\ref{sec:overview}, but since our algorithm follows and builds upon a number of previous results, we first summarize the previous results
\changed{(in historical order)}
and explain what is novel about our contributions.

\begin{enumerate}

\item \changed{Meggido, 1983~\cite{megiddo_linear}, Dyer, 1984~\cite{dyer1984linear}.  A \reviewerchange{linear-time algorithm} for linear programming in two and three dimensions.
There are two ideas from these famous prune-and-search algorithms that are used in  algorithms for geodesic centers, including ours. The first idea is to
make repeated calls to an ``oracle'' that solves the problem one dimension down.
The second idea is to eliminate constraints by pairing them up and considering the ``bisecting'' plane or line where the two constraints are equal. 
The oracle can be used to determine which 
side of the bisector contains the optimum solution, thus eliminating one 
of the two constraints.
Using techniques 
now known as cuttings or epsilon-nets, a small number of bisectors can be tested to 
eliminate a large number of constraints, resulting in a \reviewerchange{linear-time algorithm}.
}

\item Pollack, Sharir, Rote, 1989~\cite{pollack_sharir}.  An $O(n \log n)$ time algorithm to find the geodesic vertex center of a simple polygon. 
\changed{As for the linear programming algorithms described above, a main ingredient is to solve the problem one dimension down.
In particular, they develop an $O(n)$ time 
``chord oracle''
that, given
a chord of the polygon, finds the \emph{relative center} restricted to the chord
and from that, determines whether the 
center of the polygon lies to left or right of the chord.  
By applying the chord oracle $O(\log n)$ times, they limit the 
search to a subpolygon where Euclidean distances can be used.
This reduces the problem to finding 
a minimum disc that encloses some disks, which Megiddo~\cite{megiddo_spanned_ball} solved in linear time using the same approach as described above for linear programming.
}


Lubiw and Naredla~\cite{lubiw2021visibility} redid the chord oracle to handle farthest \emph{edges} instead of vertices. 

The idea used in the chord oracle algorithm is central to further developments. Expressed in general terms, 
the goal is to find a point in a domain (either a chord or the whole polygon) that minimizes the maximum distance to a %
site (a vertex or edge of the polygon). The idea is to first find what we will call a \emph{coarse cover} of the domain by a linear number of elementary regions $R$ (intervals or triangles) with an easy-to-compute \changed{convex} function $f_R$ defined on each region $R$, such that for any point $x$ in the domain, the maximum distance from $x$ to a site is the maximum of $f_R(x)$ over regions $R$ containing $x$.  Thus, the goal is to find the point $x$ that minimizes the upper envelope of the convex functions.
\changed{When the domain is a chord, the 
chord oracle finds the point $x$ in linear time using Megiddo's technique of pairing the constraints (i.e., the functions) in order to prune away a fraction of them in each round. 
When the domain is the whole polygon, 
the innovation of Ahn et al.~described in (4) below is to use similar ideas, together with $\epsilon$-net techniques, to obtain a \reviewerchange{linear-time algorithm}. 
However, finding an appropriate coarse cover of the polygon 
in linear time depends on another breakthrough, which we discuss next.
}

\item Hershberger, Suri, 1997~\cite{hershberger1997matrix}. A \reviewerchange{linear-time algorithm} to find the farthest vertex from each vertex of a polygon. This important result is 
the cornerstone of \reviewerchange{linear-time algorithm}s
{to find the geodesic diameter and center of a polygon}. 
The problem is transformed to finding row maxima in a matrix of distances between pairs of vertices.
The resulting matrix is ``totally monotone'' so the row maxima can be found with a linear number of matrix accesses using the algorithm of 
Aggarwal et al.~\cite{aggarwal1989linear}.  
Hershberger and Suri show
how to access the required distance matrix entries in amortized constant time each.

We show that Hershberger and Suri's algorithm extends to finding the farthest \emph{edge} from each vertex.

\item Ahn, Barba, Bose, De Carufel, Korman, Oh, 2016~\cite{linear_time_geodesic}.  A \reviewerchange{linear-time algorithm} to find the geodesic vertex center of a simple polygon.  
Using the algorithm of Hershberger and Suri as a starting point, they find a coarse cover of the whole polygon.  
They then use divide-and-conquer based on $\epsilon$-nets to reduce the domain to a triangle. After that, the vertex center is found using  
Megiddo-style prune-and-search techniques as described in (1) above.

Our algorithm uses a similar approach. 
One difference is that 
we give a simpler method of finding a coarse cover of the polygon by first finding 
the \reviewerchange{geodesic farthest-edge} Voronoi diagram on the polygon boundary.

Other differences are introduced in order to 
repair 
some flaws in the algorithm of Ahn et al. 
They 
recurse on subpolygons called ``$4$-cells'' that are the intersection of four half-polygons (a half-polygon is the subpolygon to one side of a chord).
However, 
the resulting range space does not in fact 
not 
have the necessary properties for finding $\epsilon$-nets.  
In addition, their step of partitioning a larger cell into $4$-cells needs repairing.  

We remedy these issues by recursing on
subpolygons that are the intersection of three 
\emph{geodesic} half-polygons, i.e., instead of cutting off the region to one side of a chord, we cut off the region to one side of a geodesic path joining two points on the boundary of the polygon.
We can then prove the requisite $\epsilon$-net properties, and we can partition larger cells into our subpolygons. 
Our approach works both for the geodesic edge center and for the geodesic vertex center, thus repairing the result of Ahn et al.
For more details, see
Section~\ref{sec:phase-II-overview}.

\item Oh, Barba, Ahn, 2020~\cite{oh2020geodesic}. This paper uses the coarse cover of the polygon from (4) above, and finds the farthest vertex Voronoi diagram inside a polygon, although not in linear time. 
Of relevance here is their first step, which is a \reviewerchange{linear-time algorithm} to find the Voronoi diagram restricted to the polygon boundary. 
We reverse the order of dependence of (4) and (5).
First, 
using the Hershberger-Suri result (3) \changed{and the coarse cover of an edge from (6) below}, we  give a considerably simpler \reviewerchange{linear-time algorithm} to find the farthest edge/vertex Voronoi diagram restricted to the polygon boundary---a problem of independent interest.  
After that, we use the boundary Voronoi diagram to produce a coarse cover of the polygon and then proceed to find the geodesic edge center.


\item Naredla and Lubiw~\cite{lubiw2021visibility}. An $O(n \log n)$ time algorithm to find the edge center of a simple polygon, based on the algorithm of Pollack et al.~described in (1) above.  In fact, the algorithm solves the more general problem of finding the center of a set of $O(n)$ half-polygons (edges being the special case where the half-polygons hug the polygon boundary).
One ingredient that we will resuse in the present paper is a linear time chord oracle for the edge center, including finding a coarse cover of a chord.

\end{enumerate}
} %




==> SoCG-1200_Phase-II.tex <==
\section{Phase II: Finding the Geodesic Edge Center}
\label{section:final_edge_center}
\label{section:PhaseII}
\label{section:Phase-II}


The first step of Phase II is 
to construct a 
\defn{coarse cover} (Definition~\ref{defn:coarse-cover}) 
of the polygon
in linear time.
\changed{As shown in Figure~\ref{fig:coarse-cover} the ``funnel'' $Y(e)$ consisting of shortest paths between a chain on $\partial P$ with farthest edge $e$ and $e$ itself can be partitioned into its shortest path map.  If the result includes trapezoids, we partition each one into two triangles\footnote{Thus our triangles are not necessarily ``apexed'' triangles as in~\cite{linear_time_geodesic}.}. 
Each triangle is bounded by two polygon chords and a segment of a polygon edge, and the distance to $e$ has the form required by Definition~\ref{defn:coarse-cover}.}
See Appendix~\ref{appendix:coarse-cover} for details.
We seek the point inside $P$ that minimizes the upper envelope of the functions of the coarse cover. 
\changed{Note that Phase I can detect if the edge center lies \emph{on} $\partial P$ so we may assume that the center is interior to $P$.}


\begin{figure}
\centering
\includegraphics[trim={0 0cm 0 0}, width=.8\textwidth]{RS_figures/edge_funnel_2-cropped.pdf}
\caption{
\changed{Constructing the coarse cover by partitioning the funnel 
$Y(e)$ (shaded) into a shortest path map from $e$ to its chain on $\partial P$ (in red).} 
}
\label{fig:coarse-cover}
\label{fig:flower}
\end{figure}


Our final divide-and-conquer algorithm follows the vertex center algorithm of Ahn et al.~\cite{linear_time_geodesic}, generalized to farthest edges, and repairing flaws in their approach.
At each step of the algorithm we have a subpolygon $Q$ whose interior contains the center together with the coarse cover elements  
\newchanged{needed to compute the edge center}
and we shrink the subpolygon and eliminate a constant fraction of the 
coarse cover.
Each recursive step takes time linear 
in the size of the subproblem (the size of $Q$ plus the size of its coarse cover).
The subpolygons we work with are
\newchanged{
\defn{$3$-anchor hulls} defined as follows. 
An \defn{anchor} is a point inside $P$, or a subchain of $\partial P$.  
A \defn{$3$-anchor hull} is the geodesic convex hull of at most three anchors.
These are weakly simple in general, but 
we only recurse on \defn{simple} $3$-anchor hulls.
}

\remove{
\defn{$3$-geodesic cells} defined as follows.
A geodesic path $\gamma$ joining two points on $\partial P$ divides $P$ into two closed weakly simple polygons that we will refer to as \defn{geodesic half-polygons}.
A \defn{$3$-geodesic cell}
of $P$ is the intersection of at most three geodesic half-polygons.
We only recurse on \defn{simple} $3$-geodesic cells. 
See Figure~\ref{fig:shatter}.
}

The algorithm has two stages.
In Stage 1
no triangle of the coarse cover contains $Q$ (this is true initially when $Q=P$), so every triangle
has a chord crossing $Q$ and we
use $\epsilon$-net techniques on the set of such chords to reduce to a smaller cell $Q'$ that is crossed by a fraction of the chords, and hence by a %
fraction of the coarse cover triangles.
Once $Q$ is contained in a triangle of the coarse cover
we show (see Lemma~\ref{lem:floating_cells_constant_size} in Appendix~\ref{appendix:Q-bounds}) that it must have constant size.
In fact, we will exit Stage 1 as soon as $Q$ has constant size.
It is then easy to reduce $Q$ to a triangle. 
After that, we switch to Stage 2, where the convexity of $Q$ allows us to use 
a Megiddo-style prune-and-search technique
\newchanged{(as Ahn et al.~do)}
to recursively reduce the size of the subproblem. 
Stage 2 is deferred to Appendix~\ref{section:constantQ}.  




\subsection{Stage 1: Algorithm for Large $Q$}
\label{section:largeQ}

Consider a subproblem corresponding to a 
\newchanged{simple $3$-anchor hull}
$Q$ with $|Q| >6$.
We give an algorithm that either finds the edge center or reduces to a subproblem with $|Q| \le 6$, which is handled by Stage 2. 
In Stage 1, 
 no triangle of the coarse cover
contains $Q$ (Lemma~\ref{lem:floating_cells_constant_size} in Appendix~\ref{appendix:Q-bounds}), so each one has a chord crossing $Q$---we denote this set of 
chords by ${\cal K}(Q)$.

To apply $\epsilon$-net techniques
we define a
\newchanged{\defn{$3$-anchor range space} as follows.
The ground set is 
a set $\cal K$ of chords of $P$,
and for each $3$-anchor hull $H$ of $P$ 
there is a range ${\cal K}(H)$ 
consisting of all chords of 
$\cal K$ that \defn{cross} $H$.
Here a chord \defn{crosses} a set  if both its open half-polygons contain points of the set.
}

\remove{
To apply $\epsilon$-net techniques
we define a
\defn{$3$-geodesic range space} as follows.
Consider a $3$-geodesic cell $G$ 
defined by geodesic paths $\gamma_1, \gamma_2, \gamma_3$.
The boundary of $G$ has a subpath of each $\gamma_i$ called a \defn{geodesic chain}.
Around $\partial G$, two consecutive geodesic chains may be joined by a subpath of $\partial P$ called a 
\defn{polygon chain} or may share a common endpoint in the interior of $P$ which we call an \defn{interior vertex} of $Q$.   
See Figure~\ref{fig:shatter}.
Observe that 
$G$ is the geodesic convex hull of its (at most three)
polygon chains and interior vertices.
\newchanged{Define a \defn{$3$-hull} to be the geodesic convex hull of at most three polygon chains and interior vertices. (These are more general since a line segment inside $P$ is a $3$-hull but not a $3$-geodesic cell.)
Define the \defn{$3$-hull range space} as follows. 
The ground set is 
a set $\cal K$ of chords of $P$,
and for each $3$-hull $H$ of $P$ 
there is a range ${\cal K}(H)$ 
consisting of all chords of 
$\cal K$ that \defn{cross} $H$.
Here a chord \defn{crosses} a set  if both its open half-polygons contain points of the set.
}
} %



The algorithm finds a constant size $\epsilon$-net of the \newchanged{$3$-anchor range space} on ${\cal K}(Q)$, 
which is 
a %
set $N \subseteq {\cal K}(Q)$ such that any \newchanged{$3$-anchor hull} %
not intersected by a chord of $N$ is intersected by only a constant fraction of the chords of ${\cal K}(Q)$---this is the important property that allows us to discard a fraction of the chords.
The set of chords $N$ forms an arrangement that partitions $Q$ into cells.
We use the chord oracle to determine which cell contains the center. We then 
add geodesic paths to 
subdivide this cell into 
a constant number of
$3$-anchor hulls
and use a \defn{geodesic oracle}
(see Appendix~\ref{appendix:geodesic-oracle})
to 
\newchanged{find which $3$-anchor hull contains the center, and to shrink it to a simple $3$-anchor hull 
$Q'$.} The algorithm recurses on $Q'$, whose coarse cover is a fraction of the size.


More details of the algorithm can be found in Appendix~\ref{appendix:Algorithm-Stage1}.  
For now, we expand on the aspects of the algorithm that differ from the approach of Ahn et al.~\cite{linear_time_geodesic}.
Instead of 
$3$-anchor hulls,
their algorithm works with \emph{$4$-cells}, 
\newchanged{formed by taking the intersection of at most four half-polygons, where a half-polygon is the part of $P$ to one side of a chord}.
The number (three versus four) is not significant, but we 
\newchanged{bound our regions by geodesics instead of chords} 
in order 
to obtain the following two results. 

\subparagraph{1.} The
\newchanged{$3$-anchor}
range space has finite VC-dimension.  This implies that constant-sized $\epsilon$-nets exist. Furthermore, there is a ``subspace oracle'' 
that allows us to find an $\epsilon$-net $N$ in deterministic linear time~\cite[Chapter 47, Theorem 47.4.3]{toth2017handbook}. For 
further 
background see Appendix~\ref{appendix:epsilon-net-overview}. 

Ahn et al.~claim that their range space 
\newchanged{(of chords crossing $4$-cells)}
has finite VC-dimension but their proof is flawed.
Our proof shows that their range space does in fact have finite VC-dimension.
\newchanged{They do not mention subspace oracles, without which their algorithm runs in expected linear time rather than deterministic linear time as claimed.}
We expand on these aspects in Section~\ref{section:epsilon-net-results} below.

\subparagraph{2.} A cell of the arrangement of $N$ can be partitioned into 
constantly many
$3$-anchor hulls.

The method used by Ahn et al.~to 
subdivide a cell of $N$ into $4$-cells by adding a constant number of chords is
incomplete.
They subdivide using vertical chords,
but their algorithm does not add enough vertical chords. 
For a counter-example, \newchanged{see %
Appendix~\ref{section:counterexample}}.
We see how to repair their partition step %
but we find 
$3$-anchor hulls
more natural.

\remove{
\begin{figure}
  \centering
  \includegraphics[width=.15\textwidth]{RS_figures/decomposition_counterexample-cropped.pdf}
  \caption{
  \changed{(a) Ahn et al.~partition a cell of the arrangement of $N$ by adding vertical chords from the endpoints and intersection points of chords $N$.  (b) A counterexample to their claim that this produces 4-cells.} 
  \old{
  Schematic outlining the problem with Ahn et al.'s proposed vertical decomposition of the polygon into 4-cells.
  The blue chords represent an $\epsilon$-net of their range space.
  Using their decomposition scheme, the polygon is not partitioned into 4-cells, contrary to their claim.}
  \anna{It would be nice to include a version of their partition figure  beside this (we should redraw to avoid copyright).}
  }
\label{fig:decomposition_counterexample}
\end{figure}
}


\subsection{$\epsilon$-Net Results for Stage 1}
\label{section:epsilon-net-results}

In this section we expand on the $\epsilon$-net results that are needed for Stage 1 of the algorithm as described above.  We also give details of the flaws in the approach of Ahn et al.~\cite{linear_time_geodesic}.
For an overview of $\epsilon$-nets as used for geometric divide-and-conquer, see Appendix~\ref{appendix:epsilon-net-overview}.
To show that $\epsilon$-nets of size $O(1)$ exist we need the following result.

\begin{lem}
\label{lem:constant_shattering_dimension}
The \newchanged{$3$-anchor}
range space has 
VC-dimension less than 259.
\end{lem}



Our proof of Lemma~\ref{lem:constant_shattering_dimension} works equally well for
\newchanged{$4$-anchor hulls}---the
bound becomes %
$372$. 
\newchanged{A $4$-cell is a special case of a $4$-anchor hull (Claim~\ref{claim:4-cell}), so}
our proof implies finite VC-dimension ($\le 372$) for the $4$-cell range space, which repairs the claim by Ahn et al.\footnote{In response to our enquiries, Eunjin Oh independently suggested a similar remedy.}.
We explain the flaw in %
their proof.
Let us refer to the set of chords intersecting a $4$-cell as a ``$4$-cell range''. 
Ahn et al.~prove that the $1$-cell range space has 
VC-dimension at most 65,535. 
They note that a $4$-cell is the intersection of four $1$-cells, and then claim in their Lemma 9.1 that
this implies finite VC-dimension for the $4$-cell range space.  As justification, they refer to 
Proposition 10.3.3 of Matousek's text~\cite{matousek2002}, which 
states 
that the VC-dimension is bounded for any family whose sets can be defined by a formula of Boolean connectives (union, intersection, set difference).
However, Matousek's proposition cannot be applied in this situation because, although a $4$-cell is the intersection of four $1$-cells,  
it is not true that 
a $4$-cell \emph{range} is the intersection of four $1$-cell \emph{ranges}.
In particular, a chord can intersect two $1$-cells, but not intersect the intersection of the two $1$-cells.  For example, a line of slope $-1$ can intersect the $+x$ half-plane and the $+y$ half-plane without intersecting the $+x,+y$ quadrant.






\begin{proof}[Proof of Lemma~\ref{lem:constant_shattering_dimension}]
We will prove that the shattering dimension is 6 and then apply the result that a range 
space with shattering dimension $d$ has VC-dimension bounded by $12d \ln{(6d)}$ (Lemma 5.14 from Har-Peled~\cite{har2011geometric}). 
For $d=6$ this is $< 259$.

For an explanation of shattering dimensions see Appendix~\ref{appendix:epsilon-net-overview}.
We must show that for
a set $\cal K$ of chords with 
$| {\cal K}| = m$, the number of distinct ranges is $O(m^6)$.
We prove that 
the range space for ${\cal K}$ is the same 
if we replace 
\newchanged{$3$-anchor hulls}
by   ``expanded $3$-anchor hulls'' that are defined in terms of $\cal K$, more precisely, 
in terms of the arrangement $A({\cal K})$
of the chords ${\cal K}$ plus the edges of $P$.
\remove{Define an \defn{interior anchor}
to be a face, edge, or vertex of 
$A({\cal K)}$, and define a \defn{boundary anchor} to be a 
\changed{polygon chain}
with endpoints in 
$V({\cal K})$, the set of endpoints of chords $\cal K$.}
\newchanged{Define an \defn{expanded anchor} to be an internal face, edge, or vertex of $A({\cal K)}$, or a 
polygon chain
with endpoints in 
$V({\cal K})$, the set of endpoints of chords $\cal K$.
An \defn{expanded $3$-anchor hull} is the geodesic convex hull of at most three 
expanded anchors.}




\begin{figure}
  \centering
  \includegraphics[width=0.7\textwidth]{RS_figures/threeGthreeAcells_4-cropped.pdf}
  \caption{
  A simple 3-anchor hull $Q$ with anchors $v_1, v_2$ and the polygon chain $c_3$. 
Solid blue chords cross $Q$, while dashed blue chords do not.  The expanded 3-anchor hull $\psi(Q)$ (lightly shaded)
has expanded anchors: $a_1$, the face in the chord arrangement containing $v_1$;
  $a_2$, the edge with $v_2$ in its interior; and
  $a_3$, the polygon chain extending $c_3$ to chord endpoints.
  The same  
  chords cross $Q$ and $\psi(Q)$.
}
\label{fig:shatter}
\end{figure}


\begin{lem}
\label{lem:anchor-ranges}
The set of ranges ${\cal R} = \{ {\cal K}(Q) \mid Q \text{ is 
a $3$-anchor hull
} \}$ is the same as 
the set of ranges
$\overline{\cal R} = \{ {\cal K}({Q}) \mid {Q} \text{ is 
an expanded $3$-anchor hull } \}$.
\end{lem}

\begin{proof}
To prove ${\cal R} \subseteq \overline{\cal R}$, consider a 
\newchanged{$3$-anchor hull $Q$.
Replace any point anchor $p$}
by the 
smallest (by containment) internal vertex, edge, or face of $A({\cal K)}$ that contains $p$.
See Figure~\ref{fig:shatter}.
Replace any 
polygon chain anchor $C$ %
by the smallest chain of 
$\partial P$ 
containing $C$ and with endpoints in $V({\cal K})$.
Let 
$\psi(Q)$ be the geodesic convex hull of these expanded anchors.  
Then $\psi(Q)$ is an expanded $3$-anchor hull that contains $Q$, and it is straight-forward to prove that 
${\cal K}(Q) = {\cal K}(\psi(Q))$
(see Claim~\ref{claim:same-crossing-chords} in Appendix~\ref{appendix:epsilon-nets}).

\remove{\begin{claim}
\label{claim:same-crossing-chords}
A chord of $\cal{K}'$ crosses $Q$ if and only if it crosses $a(Q)$,
i.e., ${\cal K}'(Q) = {\cal K}'({a(Q)})$.
\label{claim:expansions}
\end{claim}

\begin{proof} 
One direction of the proof is simple: If a chord crosses $Q$, it must cross $a(Q)$ since $Q \subseteq a(Q)$.

For the other direction we prove
that if a chord $k \in {\cal K}'$ does not cross the 
$3$-geodesic cell $Q$, 
then it does not cross the 
$3$-anchor cell $a(Q)$.
Suppose that a chord $k \in \mathcal{K}'$ does not cross $Q$. 
Then $Q$ is contained in one of the closed half-polygons, say $H$, defined by $k$.  This implies that the polygon chains and interior vertices of $Q$ are contained in $H$.  Since the corresponding anchors were defined to not cross chords of $\cal K'$, they are contained in $H$. Thus $a(Q)$, being the geodesic convex hull of sets in $H$, is also in $H$.  So $k$ does not cross $a(Q)$. 
\end{proof}
}

For the other direction, let $Q$ be an expanded $3$-anchor hull.
Replace an expanded anchor that is a face, edge, or vertex of $A({\cal K})$ by a point anchor in the interior of that face, edge, or vertex. An expanded anchor that is a polygon chain remains unchanged.
Let $\gamma(Q)$ be the
geodesic convex hull of the resulting anchors.
Observe that
\newchanged{$\gamma(Q)$ is a $3$-anchor hull and}
$\psi(\gamma(Q)) = Q$.
Thus by Claim~\ref{claim:same-crossing-chords}, ${\cal K}(Q) = {\cal K}(\gamma(Q))$.
\end{proof}

\changed{
To complete the proof of Lemma~\ref{lem:constant_shattering_dimension} we claim that the number of expanded $3$-anchor hulls of ${\cal K}$ is $O(m^6)$.
An expanded anchor may be an
internal vertex, edge, of face
of $A(\cal K)$,  of which there are $O(m^2)$ possibilities.
Otherwise, an expanded anchor is 
a chain of $\partial P$ between vertices of $V({\cal K})$, 
also with
$O(m^2)$ possibilities.
Thus the number of expanded $3$-anchor hulls 
is $O((m^2)^3) = O(m^6)$.
}
\end{proof}

\paragraph*{Subspace Oracle}

\changed{In Appendix~\ref{appendix:epsilon-nets} we prove that the $3$-anchor range space has a subspace oracle, i.e., that there is a deterministic algorithm that, given a subset ${\cal K}' \subseteq {\cal K}$ with $|{\cal K}'| = m$, computes the set
of ranges ${\cal R} = \{ {\cal K}'(Q) \mid Q \text{ is 
a $3$-anchor hull}\}$
in time 
$O(m^7)$.
The idea is 
to use Lemma~\ref{lem:anchor-ranges} and
to construct $A({\cal K}')$ minus the edges of $P$, 
and find, for each 
chord $K \in {\cal K}'$, which of the $O(m^2)$ expanded anchors in $A({\cal K}')$ intersect each side of $K$, and then, for each of the $O(m^6)$ expanded $3$-anchor hulls, eliminate the chords that have all three expanded anchors to one side, leaving the chords that cross the hull. 
}

\remove{
\begin{lem}
\label{lem:subspace-oracle}
The $3$-geodesic cell range space has a subspace oracle. 
\end{lem}

\begin{proof} We must provide a deterministic algorithm that, given a subset ${\cal K}' \subseteq {\cal K}$ with $|{\cal K}'| = m$, computes the set
$\mathcal{R}_{|{\cal K}'}$
in time $O(m^{d+1})$, where $d=6$ is the shattering dimension of the $3$-geodesic cell range space.  


In Lemma~\ref{lem:constant_shattering_dimension} we proved that 
the number of ranges in 
$\mathcal{R}_{|{\cal K}'}$ is $O(m^6)$.  Each range has at most $m$ chords in it, so the desired output, $\mathcal{R}_{|{\cal K}'}$, has size $O(m^7)$, and our goal it to compute that output in time proportional to its size.
To do this, we will basically continue the proof of Lemma~\ref{lem:constant_shattering_dimension}.
Refer back to that proof 
to see that what we
must do is find the $O(m^6)$ $3$-anchor cells $Q$, and compute for each $Q$, the set of chords of $\cal K'$ that cross it. 

To avoid dependence on $n$, we will work with the graph $G(A({\cal K'}))$
and represent each $3$-anchor cell combinatorially via its anchors. 

\anna{Here (or above?) do we need to define dummy edges?}

\old{
For a subset $\mathcal{K}' \subseteq {\cal K}$, 
define \defn{$A(\cal{K'})$} to be
the subdivision of the plane formed by the set of chords $\mathcal{K'}$ and the edges of $P$.
This is an arrangement of line segments, with the special property that all segment endpoints are on the outer face. 
Let \defn{$V({\cal K'})$} denote the endpoints of the chords in $\cal K'$.
If $\cal{K'}$ has size $m$, then
$A(\cal{K'})$ has $O(m^2)$ faces, $O(m^2)$ internal vertices and edges, and $n+2m$ external vertices and edges on the boundary of $P$. 
In particular, the external vertices are the vertices of $P$ union $V({\cal K'})$.
For our algorithms we will avoid the dependence on $n$ by working with a combinatorial version of $A(\cal{K'})$ in which each minimal chain \anurag{should this be maximal chain?}
\anna{I think minimal is correct}
along $\partial P$ with endpoints in $V({\cal K'})$
is represented by a single ``dummy edge''. 
Note that the number of dummy edges is at most $2m$.  
Let \defn{$G(A({\cal K'}))$}
denote this planar graph, which has $O(m^2)$ vertices, edges, and faces.  
}

We first compute $G(A({\cal K'}))$ as follows. 
Compute 
the arrangement of the $m$ line segments $\cal K'$ in time $O(m^2)$ \anna{cite an algorithm (Chazelle and Edelsbrunner? -- or is there a simpler more basic one?)}.  
Then, traverse the outer face of the arrangement, adding dummy edges corresponding to subchains of $\partial P$ between vertices of  $V({\cal K}')$. 
We thus compute $G(A({\cal K'}))$ in time $O(m^2)$.

Next, we enumerate all of the possible anchors: the $O(m^2)$ internal vertices, edges, and faces of $G(A({\cal K'}))$, and the $O(m^2)$ polygon chains, each represented by two endpoints in $V({\cal K'})$. 

For each of the $m$ chords $k$ of $\cal K'$ we enumerate the
anchors that lie in each of the two closed half-polygons $H$ defined by $k$.
In particular, we can traverse $G(A({\cal K'}))$ in time $O(m^2)$ to find the 
vertices, edges, and faces that lie in $H$.  We can also decide which of the $O(m^2)$  polygon chains lie entirely in $H$, based on where the endpoints lie.  This takes time $O(m^2)$ per chord, for a total of $O(m^3)$.


Finally, we can enumerate all the $O(m^6)$ choices of at most three anchors that determine a $3$-anchor cell $Q$.  For each choice we spend $O(m)$ time to find the set of chords crossing $Q$---begin with all of $\cal K'$ and eliminate chords that have all three anchors on the same side, since these are precisely the chords do not cross $Q$.
This gives us the set of chords crossing $Q$.
\end{proof}
}












==> SoCG-200_Overview.tex <==
\section{Overview of the %
Algorithm}
\label{sec:overview}

\remove{
\anna{Could skip:} The algorithm to find the geodesic edge center has two phases.  In Phase I we find the \reviewerchange{geodesic farthest-edge} Voronoi diagram restricted to the polygon boundary.  In Phase II we reduce the problem to finding a point in the polygon that minimizes the upper envelope of a linear number of easy-to-compute
convex functions each defined on a triangle inside the polygon. 
That problem is then solved using a two-stage divide-and-conquer algorithm based first on $\epsilon$-nets and then on 
prune-and-search techniques like those used in Megiddo's linear programming algorithm. 
A more detailed overview is below, but we first outline the previous work that our algorithm builds upon, and explain what is novel about our contributions.
}

\changed{Before giving the overview of our algorithm, we outline the previous work that our algorithm builds upon, and explain what is novel about our contributions.}

Pollack et al.~\cite{pollack_sharir} gave an $O(n \log n)$ time algorithm to find the geodesic vertex center of a simple polygon. 
A main ingredient is to solve the problem one dimension down.
In particular, they develop an $O(n)$ time 
\emph{chord oracle}
that, given
a chord of the polygon, finds the \emph{relative center} restricted to the chord
and from that, determines whether the 
center of the polygon lies to left or right of the chord.  
By applying the chord oracle $O(\log n)$ times, they limit the 
search to a convex subpolygon where Euclidean distances can be used.
This reduces the problem to finding 
a minimum disc that encloses some disks, which Megiddo~\cite{megiddo_spanned_ball} solved in linear time using the same approach as  for his linear programming algorithm.
The chord oracle was extended to handle farthest \emph{edges} instead of vertices by
Lubiw and Naredla~\cite{lubiw2021visibility}. 

The idea used in the chord oracle algorithm is central to further developments. Expressed in general terms, 
the goal is to find a point in a domain (either a chord or the whole polygon) that minimizes the maximum distance to a %
site (a vertex or edge of the polygon). The idea is to first find what we will call a \defn{coarse cover} of the domain by a linear number of elementary regions $R$ (intervals or triangles), 
\changed{each with an associated easy-to-compute convex function $f_R$ that captures the geodesic distance to a potential farthest edge, and with the property that
the upper envelope of the functions is 
the geodesic radius function.} %
Thus, the goal is to find the point $x$ that minimizes the upper envelope of the  functions $f_R$. 
When the domain is a chord,
the chord oracle solves this in linear time.

\changed{When the domain is the whole polygon, and the sites are vertices, 
Ahn et al.~\cite{linear_time_geodesic} gave a \reviewerchange{linear-time algorithm}.
They find a coarse cover of the whole polygon starting from 
Hershberger and Suri's algorithm~\cite{hershberger1997matrix} to find the farthest vertex from each vertex.  
They then use divide-and-conquer based on $\epsilon$-nets---their big innovation---to reduce the domain to a triangle. After that, the vertex center is found using  
Megiddo-style prune-and-search techniques 
like those used by 
Pollack et al.}

Our algorithm uses a similar approach, modified to deal with farthest \emph{edges} rather than vertices. 
Another difference is that 
we give a simpler method of finding a coarse cover of the polygon by first finding 
the \reviewerchange{geodesic farthest-edge} Voronoi diagram on the polygon boundary.
\changed{There is a \reviewerchange{linear-time algorithm} to find the geodesic farthest \emph{vertex} Voronoi diagram on the polygon boundary by Oh, Barba, and Ahn~\cite{oh2020voronoi}.
Our algorithm is considerably simpler, and the idea of using the boundary Voronoi diagram to find the center is novel.}

Other differences between our approach and that of Ahn et al. are introduced in order to 
repair 
some flaws in 
their paper.
\changed{
They use $\epsilon$-net techniques, but their range space does not have the necessary properties for finding $\epsilon$-nets in deterministic linear time. We remedy this by using a different range space, thereby repairing and generalizing their result.}


\paragraph*{Algorithm Overview}

\paragraph*{Phase I: Finding the Farthest Edge Voronoi Diagram Restricted to
the Polygon Boundary (Section~\ref{section:Phase-I})}
We first show that the \reviewerchange{linear-time algorithm} of Hershberger and Suri~\cite{hershberger1997matrix} that finds the farthest \emph{vertex} from each vertex can be modified to find the farthest \emph{edge} from each vertex.
A polygon edge $e$ whose endpoints have the same farthest edge $g$ is then part of the farthest Voronoi region of $g$.
To find the Voronoi diagram on a 
\emph{transition edge}
$e$ 
that has different farthest edges at its endpoints, we must find
the upper envelope of the coarse cover of $e$.   
\changed{We use the fact that the coarse cover of $e$ is 
constructed from two shortest path trees inside a smaller subpolygon called the \emph{hourglass} of $e$. The hourglasses of all transition edges can be found in linear time. 
In each hourglass, 
the shortest path trees allows us to construct the upper envelope incrementally in linear time---this is a main new aspect of our work.}




\paragraph*{Phase II: Finding the Geodesic Edge Center (Section~\ref{section:PhaseII})}
We first find a coarse cover of the polygon by triangles, 
each bounded by two polygon chords plus a segment of an edge, and 
each with an associated convex function that captures the %
geodesic distance to a potential farthest edge---the potential farthest edges are 
those that have 
non-empty Voronoi regions
on the boundary of $P$.
\remove{We do this by expanding the Voronoi regions on the boundary of $P$ into the interior of $P$.}
The problem of finding the edge center is then reduced to the problem of finding
the point that minimizes the upper envelope of the coarse cover functions.


To find this point we use divide-and-conquer, reducing in each step to a smaller subpolygon with a constant fraction of the coarse cover elements. 
There are two stages.
In Stage 2, once the subpolygon is a triangle, the prune-and-search approach of Megiddo's can be applied.  
In Stage 1
every coarse cover triangle that intersects the subpolygon has a boundary chord crossing the subpolygon, and $\epsilon$-net techniques are used to reduce the number of such chords, and hence the number of coarse cover elements.
Our approach follows that of Ahn et al.~\cite{linear_time_geodesic} but 
we repair some flaws---another main new aspect of our work.
Ahn et al.~recurse on subpolygons called ``4-cells'' that are the intersection of four half-polygons (a \defn{half-polygon} is the subpolygon to one side of a chord).
\newchanged{
We instead recurse on ``$3$-anchor hulls'' that are the geodesic convex hulls of at most three points or subchains of the polygon boundary.} 
These define a 
range space 
whose ground set is 
a set of chords and whose ranges are subsets of chords that cross a
$3$-anchor hull. 
We prove that our range space has finite VC-dimension, which repairs the faulty proof in Ahn et al.~for 4-cells.
Even more crucially, we give a ``subspace oracle'' that permits an $\epsilon$-net to be found in \emph{deterministic} linear time, 
\newchanged{something missing from their approach.}




==> SoCG-300_Preliminaries.tex <==
\section{Preliminaries}
\label{section:prelims}

Although our algorithm follows the pattern of the geodesic vertex center algorithm by Ahn et al.~\cite{linear_time_geodesic}, we must re-do everything from the ground up to deal with farthest edges. 
In this section we summarize the basic results we need, deferring proofs and details to the appendix.

\remove{
\anna{Give a better intro to this section, describing what each subsection is.}

We discussed a few preliminary concepts required to define the edge center in the Introduction (Section~\ref{section:introduction}).
This section discusses a few other concepts that will be  useful in describing and understanding our algorithm.
}

\subparagraph*{Notation and Definitions.}
\label{sec:notation}
A \defn{chord} of a polygon is a straight line segment in the (closed) polygon with both endpoints on the boundary, $\partial P$. 
For a point $p \in P$ and a point or line segment $s$ in $P$, \defn{$\pi(p,s)$} is the unique \defn{shortest} (or \defn{geodesic}) path from $p$ to $s$, and \defn{$t(p,s)$} is its \defn{terminal point}.
The length of $\pi(p,s)$, denoted \defn{$d(p,s)$}, is the \defn{geodesic distance} from $p$ to $s$.
For point $p$ in $P$, a \defn{farthest edge}, \defn{$F(p)$}, is an edge of $P$ that maximizes $d(p,e)$.
The \defn{geodesic radius} of $p$ is \defn{$r(p)$} $:= d(p,F(p))$.
The \defn{geodesic edge center} is a point $p \in P$ that minimizes
$r(p)$.


\remove{
\anna{This definition should take into account that 2D regions can have ties (or else refer to general position assumptions that prevent this).}
The subdivision of the polygon $P$ into regions with the same farthest edge is referred to as the \defn{\reviewerchange{geodesic farthest-edge} Voronoi diagram} and denoted \defn{${\cal V} (P)$}.
The diagram consists of two-
dimensional faces, edges (straight or curved) and vertices.
For brevity, we will sometimes refer to this as simply the `farthest edge Voronoi diagram'.
The restriction of the diagram to the boundary $\partial P$ is denoted ${\cal V} (\partial P)$.
More generally, the restriction of the diagram to a subset $S \subseteq P$, is denoted ${\cal V}(S)$.
For polygon $P$ and edge $e$, define the \defn{farthest Voronoi region of $e$} to be  
$\defn{V(e)} := \{ p \in P : \text{ for any other edge $f$, } d(p,e) \ge d(p,f) \}$.
}


\subparagraph*{General Position Assumptions.}
\label{sec:general-position}
\remove{
\begin{figure}
  \centering
  \includegraphics[width=.8\textwidth]{RS_figures/two_dimensional_bisector-cropped.pdf}
  \caption{
  Vertex $r$ 
  \changed{is equidistant from edges $e$ and $e'$ (colored red), and so is every point in the shaded region.
  The bisector between the two edges is thus two-dimensional.
  Assumption~\ref{assumption:unique_farthest_neighbor} forbids this situation.
  }
\anna{Please change the V between $e$ and $f$ so that $r$ does not lie on the bisector of the tip of the V (that confuses the situation).}
\anurag{changed}
\anna{The previous figure was much more enlightening.  This one is too complicated.  Please go back to the previous figure---just tweak the reflex vertex in the middle.}
  }
\label{fig:twod_voronoi}
\end{figure}
} %
\changed{As is standard for Voronoi diagrams of segments, e.g., see~\cite{aurenhammer2006farthest}, we use the following tie-breaking rule %
to prevent 2-dimensional Voronoi regions with more than one farthest edge.}

\remove{
To simplify the description of our algorithm, we %
\changed{make some} general position assumptions.
\anna{The next sentence is fine for a thesis, but should be skipped for a paper.}
General position assumptions are commonly used in computational geometry to deal with degeneracy in the input.
Previous algorithms on geodesic vertex centers and the corresponding Voronoi diagrams~\cite{linear_time_geodesic,aronov1993farthest,oh2020geodesic,wang2021optimal} 
used assumptions of a similar flavour.
In actual implementations, general position may be achieved by an infinitesimal perturbation of the input %
points~\cite{10.1145/77635.77639}.
Our first assumption is  common and basic.
} %




\smallskip\noindent
{\bf Tie-Breaking Rule.} 
Suppose that $p$ is a point of $P$, $e$ and $f$ are two edges that meet at reflex vertex $u$, and
$\pi(p,e) = \pi(p,f) = \pi(p,u)$. 
\changed{Let line $b$ be the angle bisector of $u$.
For $p$ not on $b$, break the tie $d(p,e)=d(p,f)$
by saying that the distance to the edge on the opposite side of $b$ is greater.}


\medskip
\changed{We make the following general position assumptions, which we claim can be effected by perturbing vertices.}

\changed{
\begin{assumptions}
\label{assumptions}
(1) No three vertices of 
    $P$ are collinear.
(2) After imposing the tie-breaking rule, no vertex is equidistant from two or more edges.
(3) No point on the polygon boundary has more than two farthest edges and no point in the interior of the polygon has more than a constant number of farthest edges.
\end{assumptions}
}
It follows that the set of points with more than one farthest edge 
is 1-dimensional, does not contain any vertex of $P$, and intersects $\partial P$ in isolated points; see Lemma~\ref{lem:1D-Voronoi-edges} in Appendix~\ref{appendix:general-position}.

\remove{
\begin{assumption}\label{assumption:no_three_points_collinear}
    No three vertices of 
    $P$ are collinear.
\end{assumption}



\begin{assumption}\label{assumption:unique_farthest_neighbor}
After imposing the tie-breaking rule, no vertex is equidistant from two or more edges.
\end{assumption}


It follows that the set of points with more than one farthest edge 
is 1-dimensional, does not contain any vertex of $P$, and intersects $\partial P$ in isolated points, see Lemma~\ref{lem:1D-Voronoi-edges} in Appendix~\ref{appendix:general-position}.
We also want Voronoi vertices to be ``nice'':




\begin{assumption}
\label{assumption:Voronoi-vertices}
No point on the polygon boundary has more than two farthest edges. No point in the interior of the polygon has more than a constant number of farthest edges.
\end{assumption}
} %


==> SoCG-400_farthest-properties.tex <==
\subparagraph*{Properties of Farthest Edges.}
\label{sec:farthest-properties}
We need the following basic ``triangle property'' (proved in Appendix~\ref{appendix:farthest-properties}) about shortest paths that cross. 

\begin{lem}
\label{lem:new_order}
Suppose the points $p$, $q$ and the edges $e$, $f$ occur in the order $p,q,e,f$ along the polygon boundary $\partial P$.
Then $d(p,e) + d(q,f) \geq d(p,f) + d(q,e)$.
\end{lem}

We then characterize what two paths to farthest edges are like, see Figure~\ref{fig:correct_orderings} and Appendix~\ref{appendix:farthest-properties}.  In particular, we generalize the farthest vertex Ordering Property~\cite{aronov1993farthest} as follows.


\smallskip\noindent
{\bf The Ordering Property.}
As $p$ moves clockwise around $\partial  P$, so does $F(p)$.






\begin{figure}
  \centering
  \includegraphics[width=0.6\textwidth]{RS_figures/possible_and_impossible_orderings_1-cropped.pdf}
  \caption{
Schematics for possible and impossible orderings of points $p$, $q$ and their farthest edges $F(p)$ and $F(q)$.  (a) The only possible ordering if $F(p) = F(q)$. %
(b),(c) The two possible orderings if $F(p) \ne F(q)$.
(d) The impossible ordering if $F(p) \ne F(q)$.  
}
\label{fig:correct_orderings}
\end{figure}







==> SoCG-500_shortest-paths.tex <==
\subparagraph*{Shortest Paths To/From Edges.}
\label{sec:shortest-paths}

As basic tools, we need \reviewerchange{linear-time algorithms} to find  shortest paths from a  given  point to all edges of the polygon, and to find shortest paths from a  given  edge to all  vertices of the polygon.
See Appendix~\ref{appendix:shortest-paths}. 



==> SoCG-600_separators.tex <==
\subparagraph*{Separators and Funnels.}
\label{sec:separators}



A geodesic path between two vertices of $P$ separates $\partial P$ into two parts, and when we focus on which vertices/edges are in opposite parts,
we call the geodesic path 
a ``separator''.
Separators, first introduced by Suri~\cite{suri1989}, are a
main tool for finding all farthest vertices in a polygon. 
In Appendix~\ref{appendix:separators} we extend the %
basic properties of separators to the case of farthest \emph{edges} and prove:
(1) 
If vertex $v$ and edge $e$
are separated by a geodesic path $\pi(a,b)$, then the shortest path from $v$ to $e$ is contained, except for one edge, in the shortest path trees of $a$ and $b$;
(2) A constant number of separators suffice to separate every vertex from its farthest edge.


==> SoCG-700_chord_oracle.tex <==
\subsection{Chord Oracles and Coarse Covers}\label{section:chord_oracle}


In this section we 
describe the chord oracle results that we need from previous work, 
and we give a unified explanation of those algorithms and our current algorithm in terms of coarse covers.
The basic function of a chord  oracle is to decide, given a chord $K$, whether the center lies to the left or right (or on) the chord.
Pollack et al.~\cite{pollack_sharir} gave a linear time chord oracle for the geodesic vertex center, 
which is at the heart of all further geodesic center algorithms.
Lubiw and Naredla~\cite{lubiw2021visibility} extended the chord oracle to the case of the geodesic \emph{edge} center. %

In both cases, 
a main 
step is 
the ``one-dimension down''
problem of 
finding 
the \defn{relative center}, which is a point $c_K$ on $K$ that minimizes the 
geodesic radius function $r(x)$.
\changed{The directions of the first segments of the paths from $c_K$ to its farthest sites determine
whether the center of $P$ lies 
left/right/on $K$
(see Appendix~\ref{appendix:oracles}).}



\remove{
\changed{Algorithms to find the [relative] center 
depend on the following convexity property of the geodesic radius function $r(x)$.}
\remove{
The algorithms to find the relative center on a chord and to find the center of a polygon depend on a crucial convexity property.
Define the \defn{geodesic radius function}, $r(x)$, for $x \in P$
to be the maximum geodesic distance from $x$ to a site (a vertex or edge). 
Thus the center is the point $x$ that minimizes $r(x)$.}
A function is \defn{geodesically convex} on $P$ if the function is convex on every geodesic path in $P$.
The following result was proved for vertex sites by Pollack et al.~\cite{pollack_sharir} and for edge sites by Lubiw and Naredla~\cite{lubiw2021visibility}.
\anna{This could go in the appendix, since we don't appeal to it from the main text.}

\begin{lem}
\label{lem:geodesically-convex}
The geodesic radius function $r(x)$ is geodesically convex.
\end{lem}

}


Algorithms to find the relative 
center of a chord 
or the 
center of a polygon
rely on a basic convexity property of the geodesic radius function (see Lemma~\ref{lem:geodesically-convex} in Appendix~\ref{appendix:oracles}), and all
follow the same pattern, which can be 
formalized via the concept of a \emph{coarse cover} of the chord/polygon. 
The idea is that 
a \emph{coarse cover} for a domain (a chord/polygon)  
is a set of elementary regions $R$ (intervals/triangles) covering the domain,
where each region $R$ has 
an associated 
easy-to-compute convex function $f_R$, 
such that the upper envelope of the $f_R$'s is the geodesic radius function.
We give a precise definition 
for the case of farthest edges
(following~\cite{lubiw2021visibility} and specialized for our Assumptions~\ref{assumptions}).

\begin{definition}
\label{defn:coarse-cover}
A \defn{coarse cover} of chord $K$ [or polygon $P$] is  
a set of 
triples $(R,f,e)$
where 
\begin{enumerate}
\squeezelist
\item 
$R$ is a subinterval of $K$ [or a triangle of $P$], $f$ is a function defined on domain $R$, and $e$ is an edge of $P$.

\item For all $x \in R$, $f(x) = d(x,e)$ and
either: $f(x) = d_2(x,v) + \kappa$ where $d_2$ is Euclidean distance, $\kappa$ is a constant
and
$v$ is 
a vertex of $P$; or
$f(x) = d_2(x, {\bar e})$, where $d_2$ is Euclidean distance and $\bar e$ is the line through $e$.

\remove{
has one of the following forms:
\begin{itemize}
\squeezelist
\item $f(x) = d_2(x,v) + \kappa$ where $d_2$ is Euclidean distance, $\kappa$ is a constant
and
$v$ is 
a vertex of $P$.

\item $f(x) = d_2(x, {\bar e})$, where $d_2$ is Euclidean distance and $\bar e$ is the line through $e$.
\end{itemize}
}


\item 
For any point $x \in K$ [or $P$], and any edge $e$ that is farthest from $x$, there is a triple $(R,f,e)$ in the coarse cover with $x \in R$. 


\end{enumerate}
\end{definition}

Condition (3) 
implies that the upper envelope of the functions of the coarse cover is the geodesic radius function. Thus the
[relative] center problem breaks into two subproblems:
(1) find a coarse cover; and (2)  find the point $x$ that minimizes the upper envelope of the coarse cover functions.
The high-level idea for solving step (2) in linear time  (for a chord or polygon domain) is to 
recursively reduce the domain (the search space) to a subinterval or subpolygon while eliminating elements 
of the coarse cover whose functions are strictly dominated by others.
\changed{As for step (1)---constructing a coarse cover---see Section~\ref{section:Phase-I} for a chord and Section~\ref{section:Phase-II} for a polygon.

We call the chord oracle in Phase II when we use divide-and-conquer to search for the center in successively smaller subpolygons.  We actually need two variations of the basic chord oracle.  
First, we need a \emph{geodesic oracle} that tests which side of a geodesic contains the center.  Secondly, we 
do not construct a coarse cover of a chord/geodesic from scratch; rather, we intersect the triangles of the coarse cover of the subpolygon with the chord/geodesic, 
thus avoiding runtime dependence on $n$.
These variations are described in Appendix~\ref{appendix:oracles}.
}

\remove{
\changed{More details on the chord oracle. 
After finding the relative center $c_K$, the last step of the chord oracle involves testing the maximum values of the coarse cover functions at $c_K$ to determine whether the center of $P$ lies left/right/on $K$.   
}

\remove{
We note that the definition in~\cite{lubiw2021visibility} allows an exception to condition (3): in case 
two triples have identical $R$ and $f$
(which implies that for all $x \in R$ the paths to two half-polygons have the same length and the the same first segment $xv$),
then we may eliminate one of them.
We do not need that exception here because we assumed that no vertex $v$ is equidistant from two or more edges (Assumption~\ref{assumption:unique_farthest_neighbor}).
}

We use a coarse cover of a chord in Phase I of our algorithm.  The chord oracle is used in Phase II. In that situation, we have a coarse cover of the polygon . . . 
where
we have a coarse cover of the polygon and are searching for a point in the polygon that minimizes the upper envelope of the coarse cover functions.  We then make calls to the chord oracle as we use
divide-and-conquer to restrict the search space to a subpolygon and
eliminate elements of the coarse cover.
As noted by Ahn et al., 
a coarse cover $\cal T$ of the polygon provides a coarse cover ${\cal T}_K$ of any chord $K$, simply by intersecting the triangles of $\cal T$ with $K$.
Substituting this for step (1) of the chord oracle 
eliminates the dependence on $n$ when the chord oracle is called during the divide-and-conquer step.
This idea is fleshed out in
\anna{Fix ref.} Section~\ref{sec:geodesic-oracle}, where we describe the type of subpolygons we recurse on, and what it means to have a coarse cover of such a subpolygon. We also generalize the chord oracle to a \emph{geodesic oracle} that tests which side of a geodesic path contains the center of the polygon.
}




==> SoCG-850_Phase-I.tex <==
\section{Phase I: Finding the Farthest Edge Voronoi Diagram Restricted to the Polygon Boundary}
\label{section:Phase-I}

\changed{Based on Assumptions~\ref{assumptions}, the boundary of $P$ consists of chains with a single farthest edge, separated by isolated points (not vertices) that have two farthest edges. 
Our goal is to find these points.}
The first step of the algorithm is to find the farthest edge from each vertex of the polygon in linear time.  To do this, we extend the algorithm of Hershberger and Suri~\cite{hershberger1997matrix} that finds the farthest \emph{vertex} from each vertex.  Details are in
Appendix~\ref{appendix:Hershberger-Suri}.
The next step is to fill in the Voronoi diagram along the polygon edges.
For an edge $ab$ where
vertices $a$ and $b$ have the same farthest edge, i.e., $F(a) = F(b)$,  all points on the edge $ab$ have the same farthest edge, by
the Ordering Property. 
An edge $ab$ with 
$F(a) \ne F(b)$ is a \defn{transition edge}. 
We will find the farthest edge Voronoi diagram on one transition edge in linear time.  To handle \emph{all} the transition edges in linear time, we will show that for each transition edge $ab$ we can restrict our attention to a subpolygon $H(a,b)$ called the \defn{hourglass} of $ab$.
(Hourglasses have been used
previously for shortest paths, Voronoi diagrams, and geodesic centers~\cite{SPT_linear,GUIBAS1989126,chazelle1989visibility,aronov1993farthest,linear_time_geodesic}.)
In Appendix~\ref{appendix:hourglasses} we show that the hourglasses of all transition edges can be found in linear time and that the sum of their sizes is linear. 

\remove{
in Section~\ref{section:functions_to_capture} we show how to find the farthest edge Voronoi diagram on a transition edge inside its hourglass in time linear in the size of the hourglass. 
For the second step, we use a coarse cover (see Section~\ref{section:chord_oracle}) of the transition edge.
}


\remove{
\anna{Keep this here? Or later?}  Later.
As explained in the Introduction, there is a \reviewerchange{linear-time algorithm} to find the farthest \emph{vertex} Voronoi diagram restricted to the boundary of a polygon due to
Oh, Barba and Ahn~\cite[Section 3]{oh2020geodesic}.
Our approach is roughly similar to theirs (with farthest edges in place of farthest vertices), but there are some significant differences.  First of all, we will use 
the Voronoi diagram on the polygon boundary to easily find a coarse cover of the polygon, whereas previous papers did things in reverse---Ahn et al.~had a more complicated way of finding a coarse cover of the polygon
which Oh et al.~then used to find the boundary Voronoi diagram. 
Another difference is that our algorithm to find the Voronoi diagram on one transition edge is considerably simpler---see Section~\ref{section:functions_to_capture} for details.
}



In this section, we show how to construct the 
farthest edge Voronoi diagram along one polygon edge $ab$ 
in time linear in the size of the polygon.
We do not assume that the polygon is an hourglass.
For purposes of description, imagine $ab$ horizontal with $a$ at the left, and the polygon interior above $ab$.
We use the \defn{coarse cover} (Definition~\ref{defn:coarse-cover}) of the edge $ab$,
which can be found in linear time (Lubiw and Naredla~\cite{lubiw_et_al:LIPIcs.ESA.2021.65}). 
Elements of the coarse cover are triples $(I,f,e)$ where $I$ is a subinterval of $ab$ and $f(x) = d(x,e)$ for any $x \in I$. 
By resolving overlaps of coarse cover intervals $I$, we find
the upper envelope of the coarse cover functions $f$, which immediately gives the Voronoi diagram on $ab$. 
This is easy if we %
sort the endpoints of the intervals $I$, but 
we cannot afford to sort. Instead, we will insert the coarse cover elements %
one by one, maintaining a list $M$ of [pairwise internally] disjoint subintervals of $ab$ together with an associated distance function $f_M(x)$. 
\changed{An efficient insertion order depends on the fact that}
\remove{When we consider  $(I,f,e)$ we will insert into $M$ the initial subinterval of $I$ in which $f(x) > f_M(x)$. 
We must be able to quickly find the left endpoint of $I$ in $M$ and to ensure that one subinterval of $I$ is all we need to add. 
This 
requires}
elements of the coarse cover of edge $ab$ are associated with edges of the shortest path trees ${T}_a$ and ${T}_b$ (that consist of the shortest paths from $a$ and $b$, respectively, to all the edges of $P$). 
We will use the ordering of the trees as embedded in the plane.



Oh, Barba, Ahn~\cite{oh2020geodesic} gave a \reviewerchange{linear-time algorithm} to find the farthest \emph{vertex} Voronoi diagram on the boundary of $P$. 
\changed{The approach is similar, but they add coarse cover elements by iterating over the sites (the vertices in their case), which involves a complicated algorithm to sweep back and forth along $M$ maintaining a shortest path to the current vertex, and a tricky amortized analysis (see~\cite[Lemma 7]{oh2020geodesic}).
Our approach is simpler and more general.} 

\remove{
Their algorithm also works by 
adding coarse cover elements to obtain the upper envelope of the distance functions.
Their coarse cover is obtained differently, and 
their algorithm is quite 
complicated---they
iterate over the sites (the vertices, in their case),  adding all coarse cover elements associated with each site.  To find the correct insertion point on $ab$, 
they sweep back and forth
maintaining a shortest path from the current point on $ab$ to the current vertex.  Their argument that updating the path costs amortized linear time depends 
on properties of the coarse cover that are not made explicit (see Lemma 7 in their paper).
Our algorithm is much simpler, both in its description and its analysis, because we
use the relationship between our coarse cover and shortest path trees, which allows us to iterate over edges of the shortest path trees rather than iterating over the sites.
}

\subsection{Farthest Edge Voronoi Diagram on One Edge}
\label{sec:one-edge-Vor}

Lubiw and Naredla~\cite{lubiw2021visibility, lubiw_et_al:LIPIcs.ESA.2021.65} constructed 
a coarse cover
(see Definition~\ref{defn:coarse-cover})
of an edge $ab$ from the shortest path trees $T_a$ and $T_b$.  They first augment $T_a$ and $T_b$ with $0$-length edges so that the paths to every 
polygon edge $e$ end with  
a tree edge perpendicular to $e$. In particular, every polygon edge corresponds to a leaf in each tree.

Direct edges of $T_a$ and $T_b$ away from their roots. 
Each edge $uv$ of $T_a \setminus T_b$ with $u \ne a$
corresponds to an \defn{$a$-side} coarse cover element $(I,f,e)$ where $e$ corresponds to the farthest leaf of $T_a$ descended from $v$.
For example, in Figure~\ref{fig:example_2_e4}, see edge $a_3$ of $T_a$ and interval $I_{a_3}$.
There are symmetrically defined \defn{$b$-side} coarse cover elements.
Each edge $uv$ of $T_a \cap T_b$ with $u$ visible from $ab$ corresponds to a \defn{central triangle} coarse cover element $(I,f,e)$ where $e$ corresponds to the farthest leaf of $T_a$ descended from $v$.
For example, see edge $a_5=b_5$ and interval $I_{a_5}$.
Each polygon edge $e$ that has an interior point visible from $ab$ corresponds to a \defn{central trapezoid} coarse cover element $(I,f,e)$ where $I$ consists of the points on $ab$ whose shortest paths to $e$ arrive perpendicularly.
For example, see edge $e_4$ and interval $I_{e_4}$.


\remove{
\changed{We first describe results of
Lubiw and Naredla~\cite{lubiw2021visibility, lubiw_et_al:LIPIcs.ESA.2021.65} on constructing 
a coarse cover
(see Definition~\ref{defn:coarse-cover})
of an edge $ab$ from the shortest path trees $T_a$ and $T_b$.} 
Direct the edges of $T_a$ and $T_b$ from the roots to the leaves (which correspond to the edges of the polygon).

\anna{Idea: Remove definition of coarse cover.  Just explain enough to get Lemma 3.  Remove figure.  Instead, put Example 2 of the algorithm.}

For any node $v$ in $T_a$ define \defn{$\ell_a(v)$} to
be the maximum length of a directed path in $T_a$ from $v$ to a  leaf node %
representing a terminal point on some 
\changed{polygon edge},
and define 
\defn{$F_a(v)$} to be that \changed{polygon edge}.
Define  \defn{$\ell_b$} and \defn{$F_b$} similarly.
These values can be computed in linear time~\cite{lubiw2021visibility}. 


Define \defn{$p_a(u)$} and \defn{$p_b(u)$} to be the parents of node $u$ in $T_a$ and $T_b$, respectively.
As noted by 
Pollack et al.~\cite{pollack_sharir}, a vertex $u$ is visible from some point on $ab$
if and only if $p_a(u) \ne p_b(u)$. 
Furthermore, note that if $u$ is visible from some point on $ab$, then extending the edge from $u$ through $p_a(u)$ reaches a point
\defn{$x_a(u)$}
on $ab$ from which $u$ is visible.
Similarly, extending the edge from $u$ through $p_b(u)$ reaches a point
\defn{$x_b(u)$}
on $ab$ from which $u$ is visible.

In order to avoid special cases,~\cite{lubiw2021visibility} assumes that  for any edge $e$ the last segment of the path $\pi(a,e)$ is orthogonal to $e$, and they add $0$-length edges to make this true. 
The extension of such a $0$-length edge is orthogonal to $e$. 
Note that, as a special case, there is a $0$-length edge added to $T_a$ at the root $a$ to account for the path (of length 0) from $a$ to the polygon edge incident to $a$.  The $0$-length edges ensure that every polygon edge is associated with a unique leaf of $T_a$.
Note that if $\pi(a,e)$ and $\pi(b,e)$ terminate at the same endpoint of $e$, then the added 0-length segment is common to both trees.

The following defines a coarse cover $\cal T$ that can be found in linear time~\cite{lubiw2021visibility}.
See Figure~\ref{fig:coarse-cover}.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\textwidth]{RS_figures/coarse_cover_elements_edge-cropped.pdf}
    \caption{
    Coarse cover elements: 
    (a) an $a$-side triangle element associated with edge $uv$;
(b) a central triangle element associated with edge $uv$;
(c) 
a central triangle element associated with $0$-length edge $uv$;
(d) a central trapezoid element %
associated with polygon edge $e$.
\anna{Drop $I_2$}
    }
    \label{fig:coarse-cover}
\end{figure}




\begin{enumerate}
\squeezelist

\item ({\bf $a$-side triangle element})
\label{list:coarse_1} 
For each directed edge $(u,v)$ in ${T}_a$ where %
\changed{$u \ne a$}, and $u$ and $v$ are both visible from $ab$, add 
$(I,f,e)$ where $I = [x_a(u), x_a(v)]$, $e = F_a(v)$ and $f(x) = d_2(x,u) + |uv| + \ell_a(v)$. 
\remove{
\item \label{list:coarse_1} For each directed edge $(u,v)$ in ${T}_a$ where \changed{$u \ne a$}, and $u$ and $v$ are both visible from $ab$, there is an associated 
{\bf $a$-side triangle} that has apex $u$ and base $I = [x_a(u), x_a(v)] \subseteq ab$. 
The associated coarse cover element is $(I,f,e)$ where $e = F_a(v)$ and $f(x) = d_2(x,u) + |uv| + \ell_a(v)$.
}
Define {\bf $b$-side triangle elements} 
symmetrically.

\item ({\bf central triangle element})
\label{list:coarse_2}
For each edge $(u,v)$ common to ${T}_a$ and ${T}_b$ with $u$ visible from $ab$, 
add $(I,f,e)$ where $I = [x_a(u), x_b(u)]$, $e = F_a(v)= F_b(v)$ and $f(x) = d_2(x,u) + |uv| + \ell_a(v)$. 

\remove{
\item \label{list:coarse_2} For each edge $(u,v)$ that is common to ${T}_a$ and ${T}_b$ where $u$ is visible from $ab$ and $v$ is not 
(i.e., $u = p_a(v) = p_b(v)$) there is an associated 
{\bf central triangle} that has apex $u$ and 
base $I = [x_a(u), x_b(u)] \subseteq ab$.
The associated coarse cover element is $(I,f,e)$ where $e = F_a(v)= F_b(v)$ and $f(x) = d_2(x,u) + |uv| + \ell_a(v)$.
}

\item ({\bf central trapezoid element})
\label{list:coarse_3}
For each
polygon edge $e$
such that the terminal points \defn{$t(a,e)$} of $\pi(a,e)$ and \defn{$t(b,e)$} of $\pi(b,e)$ are distinct,
add $(I,f,e)$ where 
$I$ is bounded by the 
two lines perpendicular to $e$ emanating from $t(a,e)$ and $t(b,e)$,
$e$ is the polygon edge and $f(x) = d_2(x,{\bar e})$ where $\bar e$ is the line through $e$. 

\remove{
\item \label{list:coarse_3} For each
polygon edge $e$
such that the terminal points \defn{$t(a,e)$} of $\pi(a,e)$ and \defn{$t(b,e)$} of $\pi(b,e)$ are distinct, 
there is a {\bf central trapezoid}
with base $I \subseteq ab$ bounded by the 
two lines perpendicular to $e$ emanating from $t(a,e)$ and $t(b,e)$---these lines are the extensions of the (possibly $0$-length) last edges of the paths.
The associated coarse cover element is $(I,f,e)$ where $e$ is the polygon edge and $f(x) = d_2(x,{\bar e})$ where $\bar e$ is the line through $e$.
}
\end{enumerate}



Note that coarse cover elements of Type~\ref{list:coarse_1} and Type~\ref{list:coarse_2} 
are associated with edges $(u,v)$ of $T_a$ and $T_b$ with at least one node visible from $ab$, and
elements of Type~\ref{list:coarse_3} %
are %
associated with %
polygon edges, 
and thus 
with leaves of $T_a$.

\remove{
\begin{obs}
\label{obs:consecutive-coarse-cover}
If $uv$ and $vw$ are edges of $T_a$ that have associated coarse cover elements $(I_1, f,e)$ and $(I_2,f',e')$, then
the right endpoint of $I_1$ is $x_a(v)$ and the left endpoint of $I_2$ is $x_a(v)$, i.e., $I$ and $I'$ appear in that order along $ab$ and intersect in a single point.  
A similar property holds for $T_b$.
\end{obs}

\begin{lem} 
\label{lem:coarse-cover-path}
Suppose edge $uv$ of $T_a$ has an associated coarse cover element 
$(I,f,F_a(v))$.
Then:

\begin{enumerate}
\item 
On the path $\pi(a,u)$ all edges except the first one have associated coarse cover elements.

\item On the path $\pi(v,F_a(v))$ let $x$ be the last vertex visible from $ab$.  All edges on $\pi(v,x)$ have associated coarse cover elements for the polygon edge $F_a(v)$.  Furthermore, if $x$ is a leaf then there is a central trapezoid associated with $F_a(v)$, and otherwise there is an edge $xy$ in $\pi(v,F_a(v))$ and it is associated with a central triangle for $F_a(v)$.
\end{enumerate}
A similar property holds for $T_b$.
\end{lem}
}

} %


\begin{lem} 
(proved in Appendix~\ref{appendix:one-edge-Vor})
\label{lem:consecutive-coarse-cover}
\label{cor:consecutive-coarse-cover}
For any edge $e$ of $P$, let $C(e)$ be the set of coarse cover elements $(I,f,e)$ for $e$.
If $C(e)$ is nonempty, then its elements correspond to a (possibly empty) path in $T_a$ directed towards a leaf, followed by a central triangle or trapezoid, followed by a (possibly empty) path in $T_b$ directed towards the root.  Furthermore, the corresponding intervals on $ab$ appear in order, are [internally] disjoint, and their union is an interval.
\end{lem}





\changed{We next construct a single tree $T$ whose edges correspond to coarse cover elements of $ab$.
Then we incrementally construct the farthest edge Voronoi diagram on $ab$ by adding coarse cover elements in a depth first search (DFS) order of $T$.
}

\remove{
\changed{This section contains the algorithm to find the farthest edge Voronoi diagram on polygon edge $ab$.  We first construct a tree $T$ whose edges correspond to coarse cover elements of $ab$.  Then we incrementally construct the farthest edge Voronoi diagram on $ab$ by adding coarse cover elements in a depth first search (DFS) order of $T$.}
}

\subparagraph*{Constructing 
tree $T$.}
Starting with $T_a$,
attach an edge for each central trapezoid element to the associated leaf vertex of $T_a$; add the path of $b$-side triangle elements for each polygon edge $e$ after the central triangle or trapezoid for $e$; and contract original edges of $T_a$ that are not associated with coarse cover elements.
See Figure~\ref{fig:example_2_e4}(right).
We give more detail of these steps in Appendix~\ref{appendix:one-edge-Vor}.
\remove{
\begin{enumerate}
\squeezelist
\item For each central trapezoid, say associated with polygon edge $e$, there is a leaf $l$
of $T$ corresponding to $e$. Attach a new edge in $T$ descending from $l$ and associate the central trapezoid with it.


\item 
For each polygon edge $e$ \changed{that has $b$-side triangles associated with it, those triangles} 
correspond to a  path $\pi$ in $T_b$, that is directed in leaf-to-root order, see Corollary~\ref{cor:consecutive-coarse-cover}.  The tree $T$ currently has an edge, say $g$, associated with the central triangle/trapezoid for $e$.  Attach the path $\pi$ at end of the edge $g$.

\item 
Finally, we delete and contract some of the original edges of $T_a$.
Delete from $T_a$ any 
original directed edge $uv$ such that $u$ is not visible from $ab$ (these edges do not have associated coarse cover elements).  By Lemma~\ref{lem:coarse-cover-path}, the result is still a tree.  Next, contract \changed{the original} edges of $T_a$ incident to $a$ (these edges also do not have associated coarse cover elements).  \changed{The edges of $T_a$ that remain in $T$ are the ones that 
have associated coarse cover elements}, i.e., all $a$-side  and central triangles.


\end{enumerate}
}
The resulting tree $T$ can be constructed in linear time and its edges are in one-to-one correspondence with the coarse cover elements. 

\begin{obs}
\label{obs:consecutive-coarse-cover-T}
If $uv$ and $vw$ are edges of $T$, then the
corresponding coarse cover intervals
$I_1$ and $I_2$
appear in that order along $ab$ and intersect in a single point. 
\end{obs}

\remove{
\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{RS_figures/example_2_for_DFS_algorithm_3_original-cropped.pdf}
\caption{
The shortest path trees rooted at $a$ and $b$ are shown in red and blue respectively.
We have constructed the diagram so that the farthest edge from points on $ab$ is either $e_4$ or $e_7$.
Tree edges not on the paths to these two edges will be ignored.
The crossover point $t$ on $ab$ is at equal geodesic distance from $e_4$ and $e_7$. Our Voronoi diagram algorithm will assign the interval $at$ to $e_4$ and $tb$ to $e_7$.
}
\label{fig:example_2}
\end{figure}
}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.43\textwidth}
        \centering
        \includegraphics[width=\textwidth]{RS_figures/example_2_for_DFS_algorithm_2_coarse_cover_for_e4_1-cropped.pdf}
    \end{subfigure}%
    \begin{subfigure}[t]{0.43\textwidth}
        \centering
        \includegraphics[width=\textwidth]{RS_figures/example_2_for_DFS_algorithm_2_coarse_cover_for_e7_3-cropped.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.13\textwidth}
        \centering
        \includegraphics[width=\textwidth]{RS_figures/Ta_and_T_example_2_1_JUST_T_rotated_1-cropped.pdf}
    \end{subfigure}
    \caption{Coarse cover elements corresponding to some (not all) edges of $T_a$ (red) and $T_b$ (blue):  (left) coarse cover elements for $e_4$; 
(middle) coarse cover elements for $e_7$;
(right) the corresponding part of tree $T$.
\changed{When {\tt Insert} compares $I_{a_4}$ to the new interval $I_{a_6}$ it finds cross-over point $t$.}
}
\label{fig:example_2_e4}
\end{figure}



\subparagraph*{DFS Algorithm for the Voronoi Diagram.}
We add the coarse cover elements following a DFS of $T$ with children of a node in clockwise order. 
We maintain a list $M$ of interior disjoint subintervals of $ab$ whose union  is an interval starting at $a$. Each subinterval in $M$ records the coarse cover element it came from. 
Define $f_M$ to be the distance function determined by the intervals of $M$.
\changed{Initially, $M$ is the single point $a$, and $f_M$ is $- \infty$.}
At the end $M$ will be the upper envelope of the coarse cover functions (though this property is not guaranteed throughout). To handle edge $uv$ of $T$ with associated coarse cover element $(I,f,e)$, we compare $f$ to $f_M$ beginning at the left endpoint of $I$. We maintain a pointer $p_u$ that gives an interval of $M$ containing this endpoint. 
The recursive routine 
{\tt Insert}$(u,p_u)$ inserts into $M$ the portions of coarse cover elements that are associated with $u$'s subtree and that define the upper envelope.  
At the top level, we call {\tt Insert}$(a,p_a)$, where $p_a$ points to $a$.


\remove{
We add the coarse cover elements one by one, ordered  according to
a depth first search of the tree $T$ in which we explore children of a vertex in clockwise order (i.e., with the most counterclockwise child first). 
We maintain a list $M$ of interior disjoint subintervals of $ab$ whose union  is an interval starting at $a$. With each subinterval in $M$ we record the coarse cover element it came from.  We define $f_M$ to be the distance function determined by the intervals of $M$.  
In the end $M$ will be the farthest edge Voronoi diagram on $ab$. 




During the depth first search of $T$, when we traverse an edge $uv$ with an associated coarse cover element $(I,f,e)$, we ensure that any part of this element that defines the final upper envelope is inserted into $M$.
(Note the subtlety that 
$M$ need not be the upper envelope of the coarse cover elements examined so far.)

In fact, the algorithm will insert only one subinterval of $I$ beginning at its left endpoint.
If all of $I$ is inserted, then the algorithm recursively continues the depth first search on vertex $v$, and otherwise the whole subtree rooted at $v$ is abandoned. 
There are two issues: correctness, which is addressed later;
and efficiency, which we discuss 
here.
In interval $I =[l,r]$ 
we must compare the distance function $f$ to the distance function $f_M$ determined by the intervals of $M$. We begin at $l$, the left endpoint of $I$.
To compare $f(l)$ with $f_M(l)$, we must locate $l$ in $M$ at unit cost. 
If $u$ is the root of $T$, then $l=a$, and we begin at the start of $M$.  Otherwise, the edge of $T$ from the parent of $u$ to $u$ has an associated coarse cover element with an interval $I'$.  
By Observation~\ref{obs:consecutive-coarse-cover-T}, the right endpoint of $I'$ is $l$.
Thus, we will store with vertex $u$ a pointer $p_u$ to the interval of $M$ that contains the right endpoint of $I'$.
This allows us to access $f_M(l)$ at unit cost.



We define a recursive routine, {\tt Insert}$(u,p_u)$ where $u$ is a vertex of $T$ and $p_u$ is a pointer into the list $M$ as described above. 
The goal is to insert into $M$ the portions of coarse cover elements that are associated with the subtree of $T$ rooted at $u$ and that determine the final upper envelope.  
Initially $M$ has a single endpoint $a$ and pointer $p_a$ points to it. At the top level we call {\tt Insert}$(a,p_a)$.
}

\remove{
\noindent
\ind{1}{\tt Insert}$(u, p_u)$
\ \ \ $u$ is a node of $T$ and $p_u$ is a pointer to an interval of $M$\\
\ind{1}1: \ind{1}{\bf for} each child $v$ of $u$ in clockwise order {\bf do}\\
\ind{1}2:\ind{2}$(I,f,e) :=$
the coarse cover element associated with the edge $uv$ of $T$.\\
\ind{1}3:\ind{2} $l :=$ left endpoint of $I$; $r :=$ right endpoint of $I$\\
\ind{4} {\bf Invariant:} $p_u$ points to an interval of $M$ that contains $l$.\\
\ind{1}4:\ind{2} {\bf if} $f(l^+) > f_M(l^+)$ where $l^+$ is just to the right of $l$  {\bf then}\\
\ind{1}5:\ind{3} replace intervals of $M$ starting at $p_u$ with a subinterval of $I$ ending at\\
\ind{6}the ``cross-over'' point $t < r$ where $f_M$ starts to dominate $f$, or at $r$\\
\ind{1}6:\ind{3} {\bf if} $f$ dominates until $r$ and $v$ is not a leaf of $T$ {\bf then}\\ \ind{1}6:\ind{4} {\bf call} {\tt Insert}$(v,p_v)$, where $p_v$ is a pointer to interval $I$ in $M$
}

\newchanged{
\medskip
\noindent
\ind{1} {\tt Insert}$(u, p_u)$
\ \ \ \# $u$ is a node of $T$ and $p_u$ is a pointer to an interval of $M$

\smallskip
\noindent
\ind{2} {\bf for} each child $v$ of $u$ in clockwise order {\bf do}\\
\ind{3} $(I,f,e) :=$
the coarse cover element associated with the edge $uv$ of $T$\\
\ind{3} $l :=$ left endpoint of $I$; \ $r :=$ right endpoint of $I$\\
\ind{3} {\bf Invariant:} $p_u$ points to an interval of $M$ that contains $l$\\
\ind{3} {\bf if} $f(l^+) > f_M(l^+)$ where $l^+$ is just to the right of $l$  {\bf then}\\
\ind{4} replace intervals of $M$ starting at $p_u$ with a subinterval of $I$ ending at\\
\ind{5}the ``cross-over'' point $t < r$ where $f_M$ starts to dominate $f$, or at $r$\\
\ind{4} {\bf if} $f$ dominates until $r$ and $v$ is not a leaf of $T$ {\bf then}\\ \ind{5} {\bf call} {\tt Insert}$(v,p_v)$, where $p_v$ is a pointer to interval $I$ in $M$
}

\remove{
\smallskip
\noindent
{\tt Insert}$(u, p_u)$
\ \ \ $u$ is a node of $T$ and $p_u$ is a pointer to an interval of $M$ \attention{ Formatting.}

\smallskip

For each child $v$ of $u$ in clockwise order: 
\begin{enumerate}
\squeezelist    

\item 
$(I,f,e) :=$
the coarse cover element associated with the edge $uv$ of $T$.  Suppose $I=[l,r]$. Our invariant is that $p_u$ points to an interval of $M$ that contains $l$.

\item if $f(l^+) > f_M(l^+)$ where $l^+$ is just to the right of $l$  then 
\begin{itemize}
\item \label{algorithm_step:premature_replace} replace the intervals of $M$ starting at $p_u$ with a subinterval of $I$ that ends at the ``cross-over'' point $t$ where $f_M$ starts to dominate $f$, or at $r$, the right endpoint of $I$, whichever comes first

\item if $f$ dominates until $r$ and $v$ is not a leaf of $T$, then call {\tt Insert}$(v,p_v)$, where $p_v$ is a pointer to interval $I$ in $M$

\end{itemize}

\end{enumerate}
}




\medskip
\noindent
{\bf Runtime:}
Each edge of ${T}$ is handled once, and causes at most one new interval to be inserted into $M$, so the total number of endpoints inserted into $M$ is $O(n)$.
We can access $f_M(l^+)$ in constant time using the pointer $p_u$. 
Then 
the endpoints of intervals of $M$ that we traverse as we do the insertion vanish from $M$. 
Thus the runtime is $O(n)$.



\smallskip
\noindent
{\bf Correctness:}
\changed{The following lemma implies that the final 
$M$ is the upper envelope of the coarse cover functions.}
\remove{
By definition, the upper envelope of the distance functions of the coarse cover elements of $ab$
is the geodesic edge radius. 
We will prove that our algorithm only discards cover elements (partially or fully) in intervals where their function value is exceeded by some other element.
The discarded parts are thus not relevant for finding the upper envelope.
At any point during the execution of the algorithm, $M$ is a list of coarse cover elements with disjoint
intervals  on $ab$ whose union is an interval starting at $a$.
All the coarse cover elements that remain in the end are part of $M$ and hence $M$ must be the upper envelope.
The following lemma completes the proof of correctness:
} %
\begin{lem}
\label{lem:DFS-correct}
The algorithm only discards pieces of coarse cover elements that do not form part of the final upper envelope.
\end{lem}



\begin{proof}
We examine the behaviour of the algorithm for edge $uv$ of $T$ with associated coarse cover element $(I,f,e)$, where $I=[l,r]$.   
We insert the subinterval $[l,t]$ into $M$ (or no subinterval). 
Because  $f(x) \ge f_M(x)$ for $x \in [l,t]$, any subintervals of $M$ that are removed due to the insertion do not determine the upper envelope, so their removal is correct. 

If we insert all of interval $I$ into $M$ and recursively call Insert$(v,p_v)$, then this is correct by induction.  
So suppose we insert a proper subinterval of $I$ or none of $I$.  
We must prove that no later part of $I$, and no element of the coarse cover associated with edges of the subtree rooted at $v$ determines the upper envelope. 
Let $t^+$ be a point just to the right of $t$ (or just to the right of $l$ if we insert no part of $I$).  Then $f_M(t^+) > f(t^+)$.
Number the polygon edges $e_1, e_2, \ldots, e_m$ clockwise from $a$ to $b$.  
Suppose that $e = e_i$, so $f(x) = d(x,e_i)$ for $x \in I$, in particular, $f(t^+) = d(t^+,e_i)$.
Suppose that 
$f_M(t^+) = d(t^+,e_k)$. 
Then $d(t^+,e_k) > d(t^+, e_i)$.  

Now consider the edges of $T$ descended from $v$ plus the edge $uv$.  Consider the corresponding coarse cover elements, $C_v$, and let $e_j$ be 
any polygon edge associated with any element in $C_v$. 
Note that the intervals on $ab$ associated with coarse cover elements of $C_v$ lie to the right of $r$, except for $I$ associated with $uv$.
We will prove that for any point $x \in ab$ to the right of $t^+$, $d(x,e_k) > d(x,e_j)$, which implies that none of the coarse cover elements in $C_v$ determines the upper envelope, nor does any part of $I$ to the right of $t$. Thus the algorithm is correct to discard them.

\changed{We first prove the result for $x = t^+$.}
If $uv$ corresponds to a central triangle/trapezoid for $e_i$
or a $b$-side triangle, then $T$ has a single path descending from $v$, all of whose edges are associated with $e_i$, i.e., $j=i$.  Otherwise, 
\changed{by the definition of
an $a$-side coarse cover element, $e_i$ corresponds to the farthest leaf of $T_a$ descended from $v$, which implies that  
}
$d(x,e_i) \ge d(x,e_j)$ for all $x \in I$, and in particular for $x=t^+$. 
Thus, in either case we have 
$d(t^+,e_k) > d(t^+, e_i) \ge d(t^+,e_j)$.

We next claim that $k < j$.  
The current $f_M$ values arise from tree edges already processed. 
These consist of: (1) edges on the path from $a$ to $u$; and (2)  edges of $T$ counterclockwise from this path.  
Edges on the path from $a$ to $u$ have coarse cover intervals on $ab$ to the left of $l$, by Observation~\ref{obs:consecutive-coarse-cover-T}.
Thus type (1) edges do not determine $f_M(t^+)$. 
By the depth-first-search order, type (2) edges have coarse cover elements corresponding to polygon edges counterclockwise from $e_j$.  Thus $k<j$.


To complete the proof of Lemma~\ref{lem:DFS-correct},
consider any point $x \in ab$ to the right of $t^+$. The clockwise ordering around the polygon boundary is $x,t^+, e_k, e_j$, so by
Lemma~\ref{lem:new_order}
and the fact that  $d(t^+,e_k) > d(t^+,e_j)$, we get $d(x,e_k) >  d(x,e_j)$, as required.  
\end{proof}



==> SoCG-save-1200-save_Phase-II.tex <==
\section{Phase II: Finding the Geodesic Edge Center}
\label{section:final_edge_center}
\label{section:PhaseII}
\label{section:Phase-II}


The first step of Phase II is 
to construct a 
\defn{coarse cover} (Definition~\ref{defn:coarse-cover}) 
of the polygon
in linear time.
\changed{As shown in Figure~\ref{fig:coarse-cover} the ``funnel'' $Y(e)$ consisting of shortest paths between a chain on $\partial P$ with farthest edge $e$ and $e$ itself is partitioned into its shortest path map.  If the result includes trapezoids, we partition each one into two triangles\footnote{Thus our triangles are not necessarily ``apexed'' triangles as in~\cite{linear_time_geodesic}.}. 
Each triangle is bounded by two polygon chords and a segment of a polygon edge, and the distance to $e$ has the form required by Definition~\ref{defn:coarse-cover}.}
See Appendix~\ref{appendix:coarse-cover} for details.
We seek the point inside $P$ that minimizes the upper envelope of the functions of the coarse cover. 
\changed{Note that Phase I can detect if the edge center lies \emph{on} $\partial P$.}


\begin{figure}
\centering
\includegraphics[trim={0 0cm 0 0}, width=.8\textwidth]{RS_figures/edge_funnel_2-cropped.pdf}
\caption{
\changed{Constructing the coarse cover by partitioning the funnel 
$Y(e)$ (shaded) into a shortest path map from $e$ to its chain on $\partial P$ (in red).} 
}
\label{fig:coarse-cover}
\label{fig:flower}
\end{figure}


Our final divide-and-conquer algorithm follows the vertex center algorithm of Ahn et al.~\cite{linear_time_geodesic}, generalized to farthest edges, and repairing flaws in their approach.
At each step of the algorithm we have a subpolygon $Q$ whose interior contains the center together with the coarse cover elements whose triangles intersect the interior of $Q$, and we shrink the subpolygon and eliminate a constant fraction of the 
coarse cover.
Each recursive step takes time linear 
in the size of the subproblem (the size of $Q$ plus the size of its coarse cover).
The subpolygons we work with are  \defn{$3$-geodesic cells} defined as follows.
A geodesic path $\gamma$ joining two points on $\partial P$ divides $P$ into two closed weakly simple polygons that we will refer to as \defn{geodesic half-polygons}.
A \defn{$3$-geodesic cell}
of $P$ is the intersection of at most three geodesic half-polygons.
\newchanged{We only recurse on \defn{simple} $3$-geodesic cells.} 
See Figure~\ref{fig:shatter}.

The algorithm has two stages.
In Stage 1
no triangle of the coarse cover contains $Q$ (this is true initially when $Q=P$), so every triangle
has a chord crossing $Q$ and we
use $\epsilon$-net techniques on the set of such chords to reduce to a smaller cell $Q'$ that is crossed by a fraction of the chords, and hence by a %
fraction of the coarse cover triangles.
Once $Q$ is contained in a triangle of the coarse cover
we show (see Lemma~\ref{lem:floating_cells_constant_size} in Appendix~\ref{appendix:Q-bounds}) that it must have constant size.
In fact, we will exit Stage 1 as soon as $Q$ has constant size.
It is then easy to reduce $Q$ to a triangle. 
After that, we switch to Stage 2, where the convexity of $Q$ allows us to use 
a Megiddo-style prune-and-search technique to recursively reduce the size of the subproblem. 
Stage 2 is deferred to Appendix~\ref{section:constantQ}.  




\subsection{Stage 1: Algorithm for Large $Q$}
\label{section:largeQ}

Consider a subproblem corresponding to a 
\newchanged{simple}
$3$-geodesic cell $Q$ with $|Q| >6$.
We give an algorithm that either finds the edge center or reduces to a subproblem with $|Q| \le 6$, which is handled by Stage 2. 
In Stage 1, 
 no triangle of the coarse cover
contains $Q$ (Lemma~\ref{lem:floating_cells_constant_size} in Appendix~\ref{appendix:Q-bounds}), so each one has a chord crossing $Q$---we denote this set of 
chords by ${\cal K}(Q)$.

To apply $\epsilon$-net techniques
\newchanged{we first define a range space.}
Consider a $3$-geodesic cell $G$ 
defined by geodesic paths $\gamma_1, \gamma_2, \gamma_3$.
The boundary of $G$ has a subpath of each $\gamma_i$ called a \defn{geodesic chain}.
Around $\partial G$, two consecutive geodesic chains may be joined by a subpath of $\partial P$ called a 
\defn{polygon chain} or may share a common endpoint in the interior of $P$ which we call an \defn{interior vertex} of $Q$.   
See Figure~\ref{fig:shatter}.
Observe that 
$G$ is the geodesic convex hull of its (at most three)
polygon chains and interior vertices.
\newchanged{Define a \defn{$3$-hull} to be the geodesic convex hull of at most three polygon chains and interior vertices. (These are more general since a line segment inside $P$ is a $3$-hull but not a $3$-geodesic cell.)
Define the \defn{$3$-hull range space} as follows. 
The ground set is 
a set $\cal K$ of chords of $P$,
and for each $3$-hull $H$ of $P$ 
there is a range ${\cal K}(H)$ 
consisting of all chords of 
$\cal K$ that \defn{cross} $H$.
Here a chord \defn{crosses} a set  if both its open half-polygons contain points of the set.
}



The algorithm finds an $\epsilon$-net of the \newchanged{$3$-hull range space} on ${\cal K}(Q)$, 
which is 
a constant-sized set $N \subseteq {\cal K}(Q)$ such that any \newchanged{$3$-hull (hence, any $3$-geodesic cell)} not intersected by a chord of $N$ is intersected by only a constant fraction of the chords of ${\cal K}(Q)$---this is the important property that allows us to discard a fraction of the chords.
The set of chords $N$ forms an arrangement that partitions $Q$ into cells.
We use the chord oracle to determine which cell contains the center. We then 
add geodesic paths to 
subdivide this cell into 
a constant number of $3$-geodesic cells and use a \defn{geodesic oracle}
(see Appendix~\ref{appendix:geodesic-oracle})
to 
\newchanged{find a simple}
$3$-geodesic cell, say $Q'$, that contains the center point. The algorithm recurses on $Q'$, whose coarse cover is a fraction of the size.


More details of the algorithm can be found in Appendix~\ref{appendix:Algorithm-Stage1}.  
For now, we expand on the aspects of the algorithm that differ from the approach of Ahn et al.~\cite{linear_time_geodesic}.
Instead of $3$-geodesic cells, their algorithm works with \emph{$4$-cells}---they use chords rather than geodesic paths to bound their cells, and they use four of them rather than three.  
The number (three versus four) is not significant, but we 
\newchanged{use geodesic cells and hulls}
to obtain the following two results. 

\subparagraph{1.} The
\newchanged{$3$-hull}
range space has finite VC-dimension.  This implies that constant-sized $\epsilon$-nets exist. Furthermore, there is a ``subspace oracle'' 
that allows us to find an $\epsilon$-net $N$ in deterministic linear time~\cite[Chapter 47, Theorem 47.4.3]{toth2017handbook}. For 
further 
background see Appendix~\ref{appendix:epsilon-net-overview}. 

Ahn et al.~claim that their range space 
\newchanged{(of chords crossing $4$-cells)}
has finite VC-dimension but their proof is flawed.
Our proof shows that their range space does in fact have finite VC-dimension.
\newchanged{They do not mention subspace oracles, without which their algorithm runs in expected linear time rather than deterministic linear time as claimed.}
We expand on these aspects in Section~\ref{section:epsilon-net-results} below.

\subparagraph{2.} A cell of the arrangement of $N$ can be partitioned into 
$O(1)$ $3$-geodesic cells.

The method used by Ahn et al.~to 
subdivide a cell of $N$ into $4$-cells by adding a constant number of chords is
incomplete.
They subdivide using vertical chords---this is why they prefer $4$-cells over $3$-cells---but their algorithm does not add enough vertical chords. 
For a counter-example, \newchanged{see %
Appendix~\ref{section:counterexample}}.
We see how to repair their partition step %
but we find 
$3$-geodesic cells more natural.

\remove{
\begin{figure}
  \centering
  \includegraphics[width=.15\textwidth]{RS_figures/decomposition_counterexample-cropped.pdf}
  \caption{
  \changed{(a) Ahn et al.~partition a cell of the arrangement of $N$ by adding vertical chords from the endpoints and intersection points of chords $N$.  (b) A counterexample to their claim that this produces 4-cells.} 
  \old{
  Schematic outlining the problem with Ahn et al.'s proposed vertical decomposition of the polygon into 4-cells.
  The blue chords represent an $\epsilon$-net of their range space.
  Using their decomposition scheme, the polygon is not partitioned into 4-cells, contrary to their claim.}
  \anna{It would be nice to include a version of their partition figure  beside this (we should redraw to avoid copyright).}
  }
\label{fig:decomposition_counterexample}
\end{figure}
}


\subsection{$\epsilon$-Net Results for Stage 1}
\label{section:epsilon-net-results}

In this section we expand on the $\epsilon$-net results that are needed for Stage 1 of the algorithm as described above.  We also give details of the flaws in the approach of Ahn et al.~\cite{linear_time_geodesic}.
For an overview of $\epsilon$-nets as used for geometric divide-and-conquer, see Appendix~\ref{appendix:epsilon-net-overview}.
To show that $\epsilon$-nets exist we need the following result.

\begin{lem}
\label{lem:constant_shattering_dimension}
The \newchanged{$3$-hull}
range space has 
VC-dimension less than 259.
\end{lem}



Our proof of Lemma~\ref{lem:constant_shattering_dimension} works equally well for
\newchanged{$4$-hulls}---the
bound becomes %
$372$.
Since $4$-cells are a subset of $4$-hulls, our proof implies finite VC-dimension ($\le 372$) for the $4$-cell range space which repairs the claim by Ahn et al.\footnote{In response to our enquiries, Eunjin Oh independently suggested a similar remedy.}.
We explain the flaw in %
their proof.
Let us refer to the set of chords intersecting a $4$-cell as a ``$4$-cell range''. 
Ahn et al.~prove that the $1$-cell range space has 
VC-dimension at most 65,535. 
They note that a $4$-cell is the intersection of four $1$-cells, and then claim in their Lemma 9.1 that
this implies finite VC-dimension for the $4$-cell range space.  As justification, they refer to 
Proposition 10.3.3 of Matousek's text~\cite{matousek2002}, which 
states 
that the VC-dimension is bounded for any family whose sets can be defined by a formula of Boolean connectives (union, intersection, set difference).
However, Matousek's proposition cannot be applied in this situation because, although a $4$-cell is the intersection of four $1$-cells,  
it is not true that 
a $4$-cell \emph{range} is the intersection of four $1$-cell \emph{ranges}.
In particular, a chord can intersect two $1$-cells, but not intersect the intersection of the two $1$-cells.  For example, a line of slope $-1$ can intersect the $+x$ half-plane and the $+y$ half-plane without intersecting the $+x,+y$ quadrant.






\begin{proof}[Proof of Lemma~\ref{lem:constant_shattering_dimension}]
We will prove that the shattering dimension is 6 and then apply the result that a range 
space with shattering dimension $d$ has VC-dimension bounded by $12d \ln{(6d)}$ (Lemma 5.14 from Har-Peled~\cite{har2011geometric}). 
For $d=6$ this is $< 259$.

For an explanation of shattering dimensions see Appendix~\ref{appendix:epsilon-net-overview}.
We must show that for
\changed{a set $\cal K$ of chords with 
$| {\cal K}| = m$, the number of distinct ranges is $O(m^6)$.}
We prove that 
the range space for ${\cal K}$ is the same 
if we replace 
\newchanged{$3$-hulls}
by   ``$3$-anchor hulls'' that are defined in terms of $\cal K$, more precisely, 
in terms of the arrangement $A({\cal K})$
of the chords ${\cal K}$ plus the edges of $P$.
Define an \defn{anchor} to be an interior face, edge, or vertex of 
$A({\cal K)}$, or a 
\changed{polygon chain}
with endpoints in 
$V({\cal K})$, the set of endpoints of chords $\cal K$.
A \defn{$3$-anchor hull} is the geodesic convex hull of at most three anchors.




\begin{figure}
  \centering
  \includegraphics[width=0.7\textwidth]{RS_figures/threeGthreeAcells_3-cropped.pdf}
  \caption{
  A simple 3-geodesic cell $Q$ defined by the red geodesics.
  \newchanged{As a $3$-hull, $Q$ is the geodesic convex hull of}
polygon chain $c_3$ (bold black) and %
points $v_1$ and $v_2$.
  Solid blue chords cross $Q$, while dashed blue chords do not.
  The $3$-anchor hull
  $\psi(Q)$ (lightly shaded) is the geodesic
  convex hull of:
  anchor $a_1$, the face in the chord arrangement containing $v_1$;
  anchor $a_2$, the edge with $v_2$ in its interior; and
  anchor $a_3$, the polygon chain extending $c_3$ to chord endpoints. 
  The same %
  chords cross $Q$ and $\psi(Q)$.
}
\label{fig:shatter}
\end{figure}


\begin{lem}
\label{lem:anchor-ranges}
The set of ranges ${\cal R} = \{ {\cal K}(Q) \mid Q \text{ is 
a $3$-hull
} \}$ is the same as 
the set of ranges
$\overline{\cal R} = \{ {\cal K}({Q}) \mid {Q} \text{ is 
a $3$-anchor hull } \}$.
\end{lem}

\begin{proof}
To prove ${\cal R} \subseteq \overline{\cal R}$, consider a 
\newchanged{$3$-hull $Q$, the geodesic convex hull of at most three points and polygon chains.}
\newchanged{Replace any point $p$}
by the 
smallest (by containment) vertex, edge, or face of $A({\cal K)}$ that contains $p$.
See Figure~\ref{fig:shatter}.
Replace any 
polygon chain $C$ %
by the smallest chain of 
$\partial P$ 
containing $C$ and with endpoints in $V({\cal K})$.
Let 
$\psi(Q)$ be the geodesic convex hull of these anchors.  
Then $\psi(Q)$ is a $3$-anchor hull that contains $Q$, and it is straight-forward to prove that 
${\cal K}(Q) = {\cal K}(\psi(Q))$
(see Claim~\ref{claim:same-crossing-chords} in Appendix~\ref{appendix:epsilon-nets}).

\remove{\begin{claim}
\label{claim:same-crossing-chords}
A chord of $\cal{K}'$ crosses $Q$ if and only if it crosses $a(Q)$,
i.e., ${\cal K}'(Q) = {\cal K}'({a(Q)})$.
\label{claim:expansions}
\end{claim}

\begin{proof} 
One direction of the proof is simple: If a chord crosses $Q$, it must cross $a(Q)$ since $Q \subseteq a(Q)$.

For the other direction we prove
that if a chord $k \in {\cal K}'$ does not cross the 
$3$-geodesic cell $Q$, 
then it does not cross the 
$3$-anchor cell $a(Q)$.
Suppose that a chord $k \in \mathcal{K}'$ does not cross $Q$. 
Then $Q$ is contained in one of the closed half-polygons, say $H$, defined by $k$.  This implies that the polygon chains and interior vertices of $Q$ are contained in $H$.  Since the corresponding anchors were defined to not cross chords of $\cal K'$, they are contained in $H$. Thus $a(Q)$, being the geodesic convex hull of sets in $H$, is also in $H$.  So $k$ does not cross $a(Q)$. 
\end{proof}
}

For the other direction, let $Q$ be a $3$-anchor hull.
Replace an anchor that is a face, edge, or vertex of $A({\cal K})$ by a point in the interior of that face, edge, or vertex. Leave the polygon chain anchors as is.
Let $\gamma(Q)$ be the
geodesic convex hull of the resulting points and chains.
Observe that
\newchanged{$\gamma(Q)$ is a $3$-hull and}
$\psi(\gamma(Q)) = Q$.
Thus by Claim~\ref{claim:same-crossing-chords}, ${\cal K}(Q) = {\cal K}(\gamma(Q))$.
\end{proof}

\changed{
To complete the proof of Lemma~\ref{lem:constant_shattering_dimension} we claim that the number of $3$-anchor hulls of ${\cal K}$ is $O(m^6)$.
An anchor may be a interior vertex, edge, or face of $A(\cal K)$, of which there are $O(m^2)$ possibilities.
Otherwise, an anchor is 
a chain of $\partial P$ between vertices of $V({\cal K})$, 
also with
$O(m^2)$ possibilities.
Thus the number of $3$-anchor hulls 
is $O((m^2)^3) = O(m^6)$.
}
\end{proof}

\paragraph*{Subspace Oracle}

\changed{In Appendix~\ref{appendix:epsilon-nets} we prove that the $3$-hull range space has a subspace oracle, i.e., that there is a deterministic algorithm that, given a subset ${\cal K}' \subseteq {\cal K}$ with $|{\cal K}'| = m$, computes the set
of ranges ${\cal R} = \{ {\cal K}'(Q) \mid Q \text{ is 
a $3$-hull}\}$
in time 
$O(m^7)$.
The idea is 
\newchanged{to use Lemma~\ref{lem:anchor-ranges} and}
to construct $A({\cal K}')$ minus the edges of $P$, 
and find, for each 
chord $K \in {\cal K}'$, which of the $O(m^2)$ anchors in $A({\cal K}')$ intersect each side of $K$, and then, for each of the $O(m^6)$ 3-anchor hulls, eliminate the chords that have all three anchors to one side, leaving the chords that cross the hull. 
}

\remove{
\begin{lem}
\label{lem:subspace-oracle}
The $3$-geodesic cell range space has a subspace oracle. 
\end{lem}

\begin{proof} We must provide a deterministic algorithm that, given a subset ${\cal K}' \subseteq {\cal K}$ with $|{\cal K}'| = m$, computes the set
$\mathcal{R}_{|{\cal K}'}$
in time $O(m^{d+1})$, where $d=6$ is the shattering dimension of the $3$-geodesic cell range space.  


In Lemma~\ref{lem:constant_shattering_dimension} we proved that 
the number of ranges in 
$\mathcal{R}_{|{\cal K}'}$ is $O(m^6)$.  Each range has at most $m$ chords in it, so the desired output, $\mathcal{R}_{|{\cal K}'}$, has size $O(m^7)$, and our goal it to compute that output in time proportional to its size.
To do this, we will basically continue the proof of Lemma~\ref{lem:constant_shattering_dimension}.
Refer back to that proof 
to see that what we
must do is find the $O(m^6)$ $3$-anchor cells $Q$, and compute for each $Q$, the set of chords of $\cal K'$ that cross it. 

To avoid dependence on $n$, we will work with the graph $G(A({\cal K'}))$
and represent each $3$-anchor cell combinatorially via its anchors. 

\anna{Here (or above?) do we need to define dummy edges?}

\old{
For a subset $\mathcal{K}' \subseteq {\cal K}$, 
define \defn{$A(\cal{K'})$} to be
the subdivision of the plane formed by the set of chords $\mathcal{K'}$ and the edges of $P$.
This is an arrangement of line segments, with the special property that all segment endpoints are on the outer face. 
Let \defn{$V({\cal K'})$} denote the endpoints of the chords in $\cal K'$.
If $\cal{K'}$ has size $m$, then
$A(\cal{K'})$ has $O(m^2)$ faces, $O(m^2)$ internal vertices and edges, and $n+2m$ external vertices and edges on the boundary of $P$. 
In particular, the external vertices are the vertices of $P$ union $V({\cal K'})$.
For our algorithms we will avoid the dependence on $n$ by working with a combinatorial version of $A(\cal{K'})$ in which each minimal chain \anurag{should this be maximal chain?}
\anna{I think minimal is correct}
along $\partial P$ with endpoints in $V({\cal K'})$
is represented by a single ``dummy edge''. 
Note that the number of dummy edges is at most $2m$.  
Let \defn{$G(A({\cal K'}))$}
denote this planar graph, which has $O(m^2)$ vertices, edges, and faces.  
}

We first compute $G(A({\cal K'}))$ as follows. 
Compute 
the arrangement of the $m$ line segments $\cal K'$ in time $O(m^2)$ \anna{cite an algorithm (Chazelle and Edelsbrunner? -- or is there a simpler more basic one?)}.  
Then, traverse the outer face of the arrangement, adding dummy edges corresponding to subchains of $\partial P$ between vertices of  $V({\cal K}')$. 
We thus compute $G(A({\cal K'}))$ in time $O(m^2)$.

Next, we enumerate all of the possible anchors: the $O(m^2)$ internal vertices, edges, and faces of $G(A({\cal K'}))$, and the $O(m^2)$ polygon chains, each represented by two endpoints in $V({\cal K'})$. 

For each of the $m$ chords $k$ of $\cal K'$ we enumerate the
anchors that lie in each of the two closed half-polygons $H$ defined by $k$.
In particular, we can traverse $G(A({\cal K'}))$ in time $O(m^2)$ to find the 
vertices, edges, and faces that lie in $H$.  We can also decide which of the $O(m^2)$  polygon chains lie entirely in $H$, based on where the endpoints lie.  This takes time $O(m^2)$ per chord, for a total of $O(m^3)$.


Finally, we can enumerate all the $O(m^6)$ choices of at most three anchors that determine a $3$-anchor cell $Q$.  For each choice we spend $O(m)$ time to find the set of chords crossing $Q$---begin with all of $\cal K'$ and eliminate chords that have all three anchors on the same side, since these are precisely the chords do not cross $Q$.
This gives us the set of chords crossing $Q$.
\end{proof}
}











